Fast and Fair Randomized Wait-Free Locks

We present a randomized approach for wait-free locks with strong bounds on time and fairness in a context in which any process can be arbitrarily delayed. Our approach supports a tryLock operation that is given a set of locks, and code to run when all the locks are acquired. A tryLock operation, or attempt, may fail if there is contention on the locks, in which case the code is not run. Given an upper bound $\kappa$ known to the algorithm on the point contention of any lock, and an upper bound $L$ on the number of locks in a tryLock's set, a tryLock will succeed in acquiring its locks and running the code with probability at least $1/(\kappa L)$. It is thus fair. Furthermore, if the maximum step complexity for the code in any lock is $T$, the attempt will take $O(\kappa^2 L^2 T)$ steps, regardless of whether it succeeds or fails. The attempts are independent, thus if the tryLock is repeatedly retried on failure, it will succeed in $O(\kappa^3 L^3 T)$ expected steps, and with high probability in not much more.

==> activesetProofs.tex <==
\section{Active Set}\label{sec:activesetProofs}



\subsection{Correctness}
We now show that Algorithm~\ref{alg:activeSet} is a linearizable implementation of an active set object. Towards this goal, we first show some basic properties of the algorithm, which will then help us specify well-defined linearization points.

%\Naama{Should require that remove(i) be called only after an insert (not concurrently).}
%\Naama{I think we don't actually need to prove linearizability for our purposes, but it shouldn't be too hard to prove.}

To ease the discussion of the algorithm's correctness, we introduce some helpful terminology. We assume that elements do not get reinserted into the active set after being removed. This is without loss of generality, as we can assign a unique id to each element when it is inserted.
We say the owner of a slot $i$ at time $t$ is the element in \code{announcements[i].owner} at time $t$. Similarly, the \emph{set} of slot $i$ at time $t$ is the set pointed at by the \code{announcements[i].set} field at time $t$.
We say an element $e$ is \emph{current} at time $t$ if there is an $i$ such that $e$ is the owner of slot $i$ at time $t$. Note that at any time $t$, there may be elements in the \code{set} field of a slot that are not current. Furthermore, the current owner of a slot at time $t$ may be null.
We let iteration $\ell$ of a call to the \code{climb} function be an iteration of the loop in the \code{climb} function where $j = \ell$. 

\begin{lemma}
	The owner of a slot $i$ never appears in the set of any slot $j$ such that $j > i$.
\end{lemma}

\begin{proof}
	Note that the \code{set} field of all slots only gets updated in the \code{climb} function. The lemma can be proven by a simple induction on the length of the execution: at the beginning of the execution, all \code{set}s are empty, and so the lemma holds. After that, note that iteration $i$ of the \code{climb} function adds the owner of $i$ to the set of slot $i$, but not any slot $j > i$. Thus, the lemma still holds after another iteration of the \code{climb} function.
\end{proof}

\begin{lemma}\label{lem:noLossClimb}
	At any point in time, the only current element that may appear in the set of a slot $i$ but not in the set of slot $i+1$ is the owner of slot $i$.
\end{lemma}

\begin{proof}
	We prove the lemma by induction on the number of times slot $i$'s set changes. The lemma trivially holds at the beginning of the execution, since the initial state of the set of all slots is empty. Assume that the lemma holds after slot $i$'s set changed at most $k$ times. Consider  the $k+1$th time it changes. Note that a set can only be changed by the CAS on Line~\ref{line:climbCAS} in the \code{climb} function. This CAS always puts in a new value that contains slot $i$'s owner plus slot $i+1$'s set. Thus, the lemma holds.
\end{proof}

\begin{lemma}\label{lem:twoCAS}
	By the end of iteration $i$ of a \code{climb} call, an owner of slot $i$ that was current at some time after the beginning of this iteration is contained in slot $i$'s set.
\end{lemma}

\begin{proof}
	Note that if one of the two CAS instances called in iteration $i$ of this \code{climb} call was successful, then the lemma holds. So, consider the case in which both CAS attempts of this iteration failed, and let $q$ be the process that executed this call. Let $R_1$ be the first time that this \code{climb} call read the set of slot $i$ on Line~\ref{line:readCurSet}, and let $R_2$ be the second time. Furthermore, let $C_1$ and $C_2$ be the first and second time (respectively) that \code{climb} call executed a CAS on \code{announcements[i].set}. Note that between $R_j$ and $C_j$, the algorithm reads the owner of slot $i$ and adds it to the new value for the subsequent CAS. If both CAS instances failed, then slot $i$'s set must have changed between $R_1$ and $C_1$, and against between $R_2$ and $C_2$. Note that slot $i$'s set changes only during the execution of a \code{climb} through a successful CAS operation. Consider the process, $p$, that executed the successful CAS operation between $R_2$ and $C_2$. $p$ must have read \code{announcements[i].set} after $R_1$, since otherwise its old value would have been outdated when it executed its CAS. Therefore, $p$ must also have read \code{announcements[i].owner} after $R_1$, and added this owner to its new value for its CAS. Therefore, $p$'s successful CAS placed an owner of slot $i$ in slot $i$'s set that was current at a time after $R_1$, and in particular, was current after the \code{climb} call of $q$ began.
\end{proof}

\begin{lemma}\label{lem:correctClimb}
	Let $t$ be the time at which a call to \code{climb(i)} terminates. There is a time $t' < t$ at which an owner of slot $i$ that was current at some time from the call to \code{climb(i)} until $t'$ is contained in the list pointed at by \code{announcements[0].set}.
\end{lemma}

\begin{proof}
	To prove the lemma, we show that after iteration $j$ of a \code{climb(i)} call, the owner of every slot $k$ such that $j\leq k \leq i$ that was current at the beginning of the $k$th iteration or later is contained in the set of slot $j$. By Lemma~\ref{lem:twoCAS}, immediately after iteration $k$, an owner of slot $k$ appears in slot $k$'s set. Furthermore, no current owner of any slot that was in the set of slot $k$ before iteration $k$ is lost by the end of the iteration. This is implied by Lemma~\ref{lem:noLossClimb}, which shows that the only current owner that can be in slot $k$'s set but not slot $k+1$'s set is the owner of $k$, and the fact that the $k$th iteration CASes in slot $k+1$'s set plus $k$'s owner into $k$'s set. Therefore, the owners get collected across iterations, so that at the end of iteration $j$ of a \code{climb(i)} call, the owner of every slot $k$ such that $j\leq k \leq i$ that was current at the beginning of the $k$th iteration or later is contained in the set of slot $j$.
\end{proof}

We can now define the linearization points of the operations.

\begin{itemize}
	\item The \code{getSet} operation linearizes at the read of the pointer to the set, on Line~\ref{line:returnSet}.
	\item The \code{insert(p)} operation linearizes at the first successful CAS on \code{announcements[0].set} that contained $p$ in the new set value.
	\item The \code{remove(i)} operation linearizes at the first successful CAS on \code{announcements[0].set} after the remove operation began whose new value did not contain the descriptor erased from slot $i$ by this \code{remove(i)}.
\end{itemize}

Note that since insert operations call \code{climb} on the slot at which they inserted an element, Lemma~\ref{lem:correctClimb} implies that there is a time during the interval of an insert operation at which the new element is present in \code{announcements[0].set}. Furthermore, recall that the set field is only ever modified with CAS operations. Therefore, the linearization point of an insert operation is well defined. Similarly, since a remove operation also calls \code{climb} on the index at which it removed an element, again by Lemma~\ref{lem:correctClimb}, there is a CAS operation during the remove operation's interval that changed \code{announcements[0].set} to a set that does not contain the removed element. Thus, the remove operation's linearization point is well defined as well.
It is easy to see that these linearization points yield a correct sequential execution, since \code{getSet} reads \code{announcements[0].set}, and both the insert and the remove operations linearize when their effect becomes visible in \code{announcements[0].set}.



\subsection{Step Complexity}

We begin by showing that the step complexity indeed depends on the point contention. That is, we define the membership point contention at a time $t$, $\kappa_t$, to be the number of elements in the active set plus the number of ongoing inserts. We claim that the step complexity of the insert operations depends on $\kappa_t$ where $t$ is a point during the insert operation's interval.

\begin{lemma}\label{lem:pointCtnSet}
	If an insert operation's successful CAS is on \\
	\code{announcements[i].owner}, then at some point $t$ during its execution, $\kappa_t$ was at least $i+1$.
\end{lemma}

\begin{proof}
	We prove this by induction on $i$. Clearly, if an insert successfully CASes its new element into slot $0$'s owner, then at the time at which it executed its CAS, there was at least 1 ongoing insertion -- its own.
	Assume that the lemma holds for an insert operation that placed its new value in slot $k$. Consider an insert operation $op$ that placed its new value in slot $k+1$. Consider the owners that $op$ saw on slots $0-k$ that made its CAS fail. Call those owners the \emph{critical owners}.
	% If all critical owners were already in their slots at the beginning of $op$'s interval, then the beginning of its interval is a point at which at $\kappa$ was least $k+2$ (these $k+1$ elements plus itself).
	
	By the induction hypothesis, for every slot $j\leq k$, the insert operation of the critical owner of slot $j$ had a point during its interval at which $\kappa$ was at least $j$. Let that point for slot $j$ be $t_j$. Consider the slot $\ell$ whose point $t_\ell$ is the latest of all such points. Then note that at $t_\ell$, the insert operations of the critical owners of all slots $\ell \leq j \leq k$ must already be pending, since otherwise their $t_j$ points would have been after $t_\ell$, contradicting the definition of $t_\ell$. Furthermore, note that $\kappa_\ell$ must include at least $\ell+1$ elements that were not inserted into slots larger than $\ell$, since we can build an execution that does not have those insertions and is indistinguishable to the process that inserted $\ell$'s critical owner. Therefore, $t_\ell$ is a point during which $\kappa$ was at least $k+1$. If $t_\ell$ is during $op$'s interval, then we are done, since $op$ itself adds another one to that total. 
	
	Otherwise, if $t_\ell$ is not in $op$'s interval, then it must have been before $op$ started, since all critical insertions were complete by the end of $op$'s interval. In this case, all insertions of the critical owners that $op$ encountered must have already started at the time at which $op$ started, and since $op$ saw these owners, their removals did not yet happen. Therefore, the invocation of $op$'s interval is a point at which $\kappa \geq k+2$.
\end{proof}

Note that the remove operation starts at the same slot as its corresponding insertion placed its element. Therefore, the remove operation traverses the same amount of slots as its corresponding insertion, which, by Lemma~\ref{lem:pointCtnSet}, is proportional to the point contention $\kappa$ during the insertion. If the active set is used as a membership tracker wherein the insert and remove operations signify the beginning and end of an operation in some external system (as it is used in our lock algorithm), the insert operation's point contention is also a valid point contention for the overall operation in the external system.

We now briefly discuss the step complexity of the rest of the active set algorithm. Of interest is the \code{climb} function, which must make copies of the \code{set} fields of each slot. If we assume that it always makes deep copies, then we can consider each such copy to take time linear in the size of the set being copied. Since the sets never contain more than $\kappa_t$ elements at any time $t$, we can bound this time by the point contention as well. Therefore, the insert and remove operations take $O(\kappa^2)$ steps. However, we can improve the time it takes to copy each set into the new one by implementing each set as a linked list, and \emph{cons}ing the new element into the front of the list. More precisely, the \code{set} field of a slot $i$ points to the head of the linked list representing its set. When executing the $i-1$th iteration of a \code{climb}, a process creates a new node containing the owner of $i-1$ and makes it point to the head of slot $i$'s list. It then swings slot $i-1$'s \code{set} pointer to point to the newly added head. Notice that in this approach, the set of slot $i$ is not changed in iteration $i-1$, since the linked list starting at the pointer from slot $i$'s \code{set} field still does not contain the owner of $i-1$. Using this technique for maintaining and updating the sets, each iteration of the \code{climb} function takes constant time, and therefore, by Lemma~\ref{lem:pointCtnSet}, the total time for an insert or remove operation is $O(\kappa)$.

The \code{getSet} takes constant time, as it simply returns a pointer to the set. Note that this is still an atomic read of the set, since the set itself is never changed; for any $i$, every time \code{announcements[i].set} is changed, its pointer is simply swung to a new location.

\paragraph{Space Complexity.} The \code{announcements} array has $C$ slots, each of which can point to a set of at most $C$ elements. However, these $C$ elements are shared among the sets. In particular, each element only has one copy. Still, garbage collection must by employed to ensure the safe release of elements that have been removed from the set. This can be done using the wait-free reference counting presented in~\cite{anderson2021concurrent}, yielding a total space usage of $O(C^2)$. If there are many active set objects in the same system (as is the case in our lock algorithm) the total space is $C$ per active set object in the system plus $O(C^2)$. 
%Using the wait-free reference counting presented Since deep copies of these sets are made, we must employ some garbage collection mechanism to prevent unbounded space usage. \Naama{To be continued.}

==> algorithm.tex <==
\section{Lock Algorithm}

We now present an algorithm for mutual exclusion that is \emph{lock-free}, \emph{fair}, and takes time proportional to the length of a critical section. More specifically, every process has a thunk to execute (representing its critical section), which is specified in a \emph{descriptor}. We achieve \emph{lock-freedom} by having processes help the current holder of the lock execute its thunk, at which point it can be removed from the lock. Thus, we require processes using our algorithm to have \textit{idempotent} thunks. As shown in Section~\ref{sec:idempotence}, this requirement is not too restrictive, since any code based on \oread{}, \owrite{}, and \cam{} can be made idempotent with constant overhead.  Our algorithm ensures that if all processes' thunks are idempotent, then the execution of the thunks is safe; a thunk's execution appears it executed
exactly once, and is not interleaved with any other thunk on the same lock.  

The algorithm proceeds in \emph{\op{}s} to grab a common lock using a \texttt{tryLock}.    In addition to the lock, \texttt{tryLock} is passed an idempotent thunk to run if the lock is successfully acquired. Each \op{} returns either \emph{true} or \emph{false}, corresponding to success or failure in acquiring the lock and running the thunk.  
At any point in time, at most one \op{} can hold the lock and execute its thunk.   This does not preclude two overlapping \op{}s 
both succeeding, as long as their locked portion does not overlap.
If an \op{} returns false, the process may retry.
We assume, without loss of generality, that each attempt is executed with a unique descriptor. Therefore, we sometimes refer to attempts and descriptors interchangeably. 
Furthermore, we enforce the following notion of \emph{fairness} in the execution: if the point contention of the \op{} of a descriptor $d$ is $\kappa$, then $d$ will succeed with probability at least $\frac{1- \epsilon}{2\kappa}$, where $\epsilon$ is an arbitrary small constant defined below.  
% $p$'s \op{} to grab the lock contends with $t$ others, then $p$ has a probability of $1/t+1$ to grab the lock in this \op{}.

The pseudocode is presented in Algorithm~\ref{alg:single-lock}. 
The algorithm relies on the \emph{write-with-max (wwm)}  primitive~\cite{shun2013reducing} to allow processes to have a fair chance of acquiring the lock, by having them compete with priorities drawn uniformly at random . %Intuitively, each \op{} has two phases; first, the initiating process picks a \emph{priority} uniformly at random, and executes a  \wwm{}with its priority on a global location called the \texttt{docket}. Intuitively, the \texttt{docket} holds the descriptor that will be next to acquire the lock. If an \op{} $a$ has the highest priority of all current \op{s}, then it will succeed in placing itself in the \texttt{docket}, and will be next in line for the lock.
%
In more detail, 
a global announcement array \texttt{announce} holds the descriptors of all processes that are currently \op{}ing to grab the lock, allowing all processes to see each other's descriptors and help execute the corresponding thunks when necessary. To determine which process is currently holding  the lock and which should be the next to grab it, two slots are maintained with pointers into the announcement array. The \live{} slot stores a pointer to the descriptor  of the process currently holding the lock. Before changing the pointer in \live{}, a process must ensure that  the descriptor pointed to has been executed to completion. The second slot is called the \docket{}, and intuitively specifies which process is next to grab the lock. Processes use \emph{priorities} to compete on inserting their own pointer into the \docket{}.

Before a process $q$ begins an \op{}, it must choose a random \emph{priority} $\rho$, and write its descriptor into \texttt{announce}$[\rho]$. The announcement array has $k$ slots (and, accordingly, the range of priorities is $k$). 
The probability of collision is $\epsilon \leq k/P$ and to decrease this probability, $k$ can be chosen to be $>> P$, where $P$ is an upper bound on the possible point contention in any execution.    
This is the same $\epsilon$ that appears in the overall success bound.
%Since a process's priority is the index in which its descriptor is written in the announcement array, we use \emph{priority} and \emph{pointer} interchangeably in the rest of this description.
%\Naama{Might want to change this description to rely less on the announcement array and its specific size, and instead say that we use  \wwm{}on the docket, and write in a pointer to the descriptor.}

After announcing its descriptor, $q$ now uses a \textsc{wwm} to \op{} to write its priority into the \docket{}. From this point on, all processes execute the same code to complete an \op{}, regardless of their descriptor's priority and whether or not their \wwm{} succeeded. In particular, all processes help execute the thunk of the current holder of the lock and ensure that progress is being made by helping a new priority get written into \live{}. 

More specifically, a process $q$ executes this helping mechanism by trying to copy the value currently written in the \docket{} into the \live{} slot using a CAS. Before doing so, however, it reads the value $\ell$ that is currently in the \live{} slot, and helps to execute the descriptor it points to. Since we require that all thunks be \emph{idempotent}, this is safe even if several processes execute this descriptor.
Furthermore, $q$ ensures that $\ell$ is not the value still written in the \docket{}, by using a CAS with $\ell$ as the old value to try to clear the \docket{}'s contents. This CAS prevents the \docket{} from being forever blocked by a single descriptor that happened to pick a high priority. 
%$\ell$ could simultaneously be in the \live{} and \docket{} slots if its priority was so high that competing processes did not overwrite it with their own priorities using write-with-min. Clearing the \docket{} in this way ensures that $\ell$ cannot block others from having a fair chance at grabbing the lock in the future.

The process $q$ executes this helping mechanism three times; twice are needed to guarantee that by the end of $q$'s \op{}, some process that wrote its priority into the \docket{} \emph{after $q$ started its \op{}} has successfully grabbed the lock. This is important to ensure that $q$'s \op{} to grab the lock is successful if and only if its descriptor gets executed. That is, it prevents the possibility that $q$'s priority  gets written into \live{} after $q$ completes its \op{}. Finally, after helping to move a value from the \docket{} to the \live{} slot twice, $q$ executes the descriptor pointed to by the \live{} slot and clears the \docket{} one more time, again ensuring that if its own priority did get written into the \live{} slot, then it will get executed before $q$ terminates.\footnote{The number of rounds can be reduced in most cases by checking various outcomes, but we prefer to keep it simple.}

%\Naama{Questions about idempotence: How easy is it to make something idempotent, how much overhead does it  introduce? Is it common for a piece of code to be idempotent by itself, but not be safe in a concurrent setting with other code? (Answer: we show (possibly in a different paper) how to make any code idempotent with constant overhead. To be safe in a concurrent setting, you have to know what other concurrent code might be run. With locks and idempotent code, the only code you might be concurrent with is copies of yourself.)}
%
%\Naama{Define our contention in terms of point contention.}
%
%\Naama{TODO: change clearing to be after helping, in its own unlock() function}


\renewcommand{\figurename}{Algorithm}
\begin{figure}[h]
\begin{lstlisting}[multicols=2]
struct announce{
	Descriptor* desc;
} announce[k];
struct Descriptor{
	Thunk thunk;
	bool done;	}
	
class Lock{
	int docket, live;
	
	void help(int index){
		CAS(&docket, index, 0); @\label{line:tryClear}@ 
		Descriptor desc = Read(&announce[index]);
		runThunk(desc.thunk);
		desc.done = true;	}
	
	void compete(){
	@{\color{red} //}@for (int i = 0; i < 3; i++){
			int @$\ell$@ = Read(&live); @\label{line:rdlive}@
			int d = Read(&docket); @\label{line:rddocket}@
			help(@$\ell$@); @\label{line:help1}@
			CAS(&live, @$\ell$@, d); @\label{line:liveCAS}@		}	}
}

int findSlot(Thunk my_thunk){
	int priority = random(1, @$k$@);
	Descriptor my_descriptor = {my_thunk, false};
	if CAS(announce[priority], NULL, &my_descriptor){
		return priority;	}
	return -1.	}
	
int clearSlot(int index){
	announce[index] = NULL;	}
	
bool check(int index){
	return Read(announce[index]->done);	}
	
bool tryLock(Thunk my_thunk, Lock @$\ell$@) {
	@{\color{red}  compete();}@
	int priority = findSlot(my_thunk);
	if (priority == -1) { return false; }
	@$\ell$.\wwm@(&docket, priority);
	@{\color{red} for (int = 0; i<3; i++)\{}@
	@$\ell$@.compete(); @{\color{red} \} }@
	bool res = check(priority);
	clearSlot(priority);
	return res;	
}
\end{lstlisting}
\caption{Lockless Lock.   The \texttt{tryLock}$(f, l)$ will attempt to acquire the lock $l$ and run the thunk $f$ if successful.
It returns a boolean indicating whether it was successful.}
	\label{alg:single-lock}
\end{figure}

\subsection{Analysis}

It is easy to see that each \op{} takes time proportional to the length of  a thunk; each \op, regardless of success or failure, executes a constant number of steps and helps run three thunks.

We now briefly sketch the proofs of safety and fairness of the lock algorithm, and present the full proofs in Appendix~\ref{sec:single-lock-proof}.

\begin{theorem}
	The algorithm presented in Figure~\ref{alg:single-lock} ensures the following mutual exclusion safety conditions.
\begin{enumerate}
	\item A thunk gets executed if and only if its \op{} returns true,
	\item At most one thunk holds the lock at any time, and
	\item A thunk cannot get executed at time $t$ if it is not holding the lock at $t$.
\end{enumerate}	
\end{theorem}

We define the descriptor `holding the lock' at time $t$ as the descriptor that is written in the \texttt{live} slot of the lock at time $t$. Clearly, there can only be one at a time. Only a descriptor holding the lock gets help (Line~\ref{line:help1}), and a thunk execution is only called from the help function. Thus, any descriptor that never held the lock can never have its thunk executed. We note that a descriptor is only ever removed from the \texttt{live} slot by a CAS executed on Line~\ref{line:liveCAS}, after a process returns from the help function. Since the help function always executes a thunk to completion, a descriptor that was on the \texttt{live} slot at some point can only get removed if its thunk has been executed to completion at least once. Relying on the idempotence property, this ensures safety. 

Finally, we argue that a thunk must get executed before its \texttt{tryLock} returns by showing that repeating the help procedure 3 times guarantees that it has helped some descriptor that was put on the docket after its \wwm. Thus, if it is going to get its thunk executed, it must have already done so.

We now focus on the fairness bound. For that purpose, we introduce a few definitions to aid the discussion of how different attempts interact with each other in an execution. In particular, we define special instructions that we say are \emph{associated} with a given \op{} executed by some process $q$. These instructions happen during the \op's execution interval, but are not necessarily executed by $q$ itself. Intuitively, these can be seen as \emph{milestones} in the progress of a descriptor's attempt. 
We consider read-CAS pairs in which the CAS was successful and executed on the \texttt{live} slot  on line~\ref{line:liveCAS}, and the read was the read on line~\ref{line:rdlive} that provided the CAS's new value. We call the first such read-CAS pair that occurs after a descriptor $d$'s \wwm{} $d$'s \emph{critical} read-CAS pair. Individually, we call them $d$'s \firstcritread{} and \firstsuccCAS.  Additionally, the first CAS on the \docket{} whose old value was read from \live{} after $d$'s \firstsuccCAS{} is called $d$'s \emph{\assocClear{}}. Note that an \assocClear{} does not have to be a successful CAS.

We show that these particular instructions and their timing with respect to the progress of other concurrent \op{s} will be crucial in determining the success or failure of the \op. For this purpose, we consider sub-intervals  of an \op's execution.

\begin{definition}
	A descriptor $d$'s \emph{\dangerInt{}} is the interval between its \wwm{} and its \firstcritread{}.
\end{definition}

\begin{definition}
	A descriptor $d$'s \emph{\activeInt{}} is the interval between its \wwm{} and its \assocClear{}. \Naama{Need to consider not the conflict interval but the `active' interval; until that process terminates. Then the 3 iterations is good enough to reduce our bounds to $1/C$.}
\end{definition}

We then say that a descriptor $d$ \emph{threatens} a descriptor $d'$ if $d$'s \activeInt{} overlaps with $d'$'s \dangerInt. Note that this relationship is asymmetric; $d$ can threaten $d'$ without being threatened itself. 
Intuitively, to capture the fairness of the algorithm, we show that a descriptor $d$ will fail only if some other descriptor with a higher priority threatens $d$'s \dangerInt{}. Furthermore, we show that the set of priorities that a given descriptor $d$ competes against is always uniform and i.i.d., and its size is at most twice the point contention that $op$ experiences. Therefore, if $d$ found an announcement slot, $d$'s probability of success is simply the probability that its priority is the highest of at most $2\kappa$ uniform, independent, and identically distributed random variables (i.e. $\geq \frac{1}{2\kappa}$), where $\kappa$ is the point contention $d$ experiences in the given schedule.

\Naama{With the new helping done before the \wwm, we have that \emph{Given 3 attempts $a,b,c$, where $a$ threatens $b$ and $c$ starts after $a$ terminates, $c$ and $b$ cannot threaten one another.} Actually, we have this even without the helping before, I think, just by helping 3 times (once after your \activeInt{} was over), because $a$ would have helped $b$ finish its \activeInt{} before terminating. In that case, with an adversary that only gets info on an attempt's priority after it terminates, that info cannot be used to affect anything.}

To show that $2\kappa$ threateners exist, we show that:

\begin{lemma}\label{lem:early-end-body}
	If a descriptor $d$ threatens a descriptor $d'$ then $d$'s \activeInt{} ends at the same time as or earlier than $d'$'s \activeInt.
\end{lemma}

This prevents the same process from making more than two attempts that contend with any one descriptor, and allows us to find two points during $d$'s execution (namely, the beginning and end of its \dangerInt), at which all its threateners must overlap with it. The proof of this lemma makes use of the `milestones' defined for each attempt; we show that a descriptor $d$ whose \firstcritread{} is before another descriptor $d'$'s \firstcritread{} (i.e. $d$ threatens $d'$) must accomplish all of its milestones at the same time as or before $d'$'s corresponding milestones.

\paragraph{Space bound.} We note that the amount of space the lock requires is dominated by  the announcement array, whose size affects the probability of collisions in this algorithm. However, aside from the announcement array, each lock only maintains two pointers; the \texttt{docket} and the \texttt{live} slots. In a system with multiple such locks, the announcement array can be shared. If there are only at most $P$ processes in the system at any time, then the probability of collisions is bounded regardless of how many locks share the array.


%Furthermore, we show that the algorithm provides efficient and fair access to the lock for all participating processes. In particular, we show that the probability for a given \op{} $a$ to succeed is $1/c$ where $c$ is the amount of contention that $a$ experiences, assuming that the \texttt{findSlot} function succeeded for this attempt. We separately bound the probability  of success for \texttt{findSlot} as a function of $k$, the size of the announcement array. 



==> applications.tex <==
\section{Applying Our Lockless Lock}

\subsection{Node Updates in a Graph}

Consider a graph with $n$ nodes and max degree $\Delta$. We show how to implement insert and delete operations into such a graph in a lock-free manner using our lock. \Naama{Or any updates (for example on a communication graph, do operations on nodes based on your state and neighbor's state (passing money to my neighbor, etc.)).}
The idea is as follows. We associate a lock with each node \Naama{or with each pointer of each node}. To insert or delete node $n$, acquire the lock of each of its neighbors, as well as its own lock. Now modify the relevant pointers as needed. This generally involves swinging the pointers either to \texttt{null} or to point to one of the nodes we have locked. These pointer swings can be done in an idempotent manner  by executing them with a CAM.

Thus, to insert or delete a node $n$, a process $p$ only needs to contend with the processes that are modifying nodes in $n$'s neighborhood. If we designate one \emph{owner} process per node, then modifying a node can only contend with $\Delta$ other processes.  \Naama{Discuss examples of where it makes sense to have an owner node (e.g. in our RSQ reclamation scheme, we designate the process that replaced a node with a newer version as the owner of that node for collection).} Thus, the write-with-min for each lock can be implemented with the universal construction with only $\Delta$ time and space.

GraphLab does this (grab a lock for all your neighbors).

Other applications: balanced tree

If no owner, recognize that the person who grabbed the locks wanted to do the same operation as you, and you help them. Don't take another empty slot in this case.

==> idempotent.tex <==
\section{Idempotence}\label{sec:idempotence}

% In this section we discuss running code inside a lock so that it is safe for other processes to help run the code.  We leverage the work of Turek et al.~\cite{turek1992locking}, but extend it in an important way.   In particular, their approach assumes no other processes, beyond the helpers, race with the lock code.   Here, we allow the lock code to race with other code---i.e., the code within the lock may access parts that aren't protected by the lock, in which other processes (beyond the helpers) can concurrently read and update locations.  The code within the lock will appear as if it ran just once in some valid interleaving with these other processes.     Thus, this allows code that only needs to protect some parts with a lock, but can safely race in other parts while still holding the lock.


% The code inside the lock can be wrapped in a thunk, as described in Section~\ref{sec:model}.  In addition to the process that acquires the lock with the intent of running the thunk, any number of other processes might help run this thunk.  Our goal is to ensure that the thunk appears to have run only once. For this, we use the notion of \emph{idempotence}, which roughly means that a piece of code that is applied multiple times appears as if was run once~\cite{idempotence02,idempotence13,idempotence12,ben2019delay}.  In this section we define it formally for our purposes, and show how to achieve this property for general code.

% \paragraph{Defining Idempotence.}

% A thunk $T$ specifies a sequence of steps, or memory operations, $S_t$. A step $s \in S_t$ is said to be \emph{a step for thunk $T$}, regardless of which process executes it.
% A \emph{run} of a thunk $T$ is the sequence of steps taken by \emph{a single process} to execute or help execute $T$.  
% %Here we are only considering memory operations in the steps.  
% An \emph{instantiation} of a thunk is a sequence of steps executed for it in some given history $H$, potentially by several different processes, such that these steps have the same arguments and return values as a correct (possibly partial) single run of the thunk.  That is, the steps in an instantiation of $T$ must be a prefix of the sequence $S_t$, but may be taken from several different runs.
% %The steps of a thunk $T$ in a given instantiation do not have to be executed by the same process---i.e., it can be taken from parts of multiple runs.  \Naama{Not sure if this is clear enough. We don't want to allow repetitions of steps. We also want it to make sense if there are any if statements in the thunk, then looking at the instantiation with the arguments and return values of the memory operations, we should have followed the right execution path.}

% \begin{definition}[Idempotence]
% \label{def:idempotence}
% 	A thunk $T$ is idempotent if in any valid history $H$,
% %  A thunk $T$ is idempotent if given any number of runs, possibly concurrent with each other and other procedures, then for all valid histories $H$ with at least one finished run of $T$:
% \begin{enumerate}
% \item
%   there exists a valid instantiation $H'$ of $T$ that is a (possibly empty) subsequence of all operations from
%   runs of $T$ in $H$,
% \item
%   if there is a finished run of $T$ (response on $T$), then the last step of the first such finished run must be the end of $H'$,
% \item
%   all memory operations for $T$ in any of its runs in $H$ that are not in $H'$ have no effect.
% \end{enumerate}
% \end{definition}
% %\Naama{H' is a history potentially from different threads, but only one "copy" of each instruction of T... Consider defining a set $\mathcal{H}$ of histories we can pick H' from. Consider also defining the projection of H onto instances of T, and get rid of all of that minus H'.}
% The definition essentially states that the combination of all runs of a thunk $T$ is equivalent to having run
% $T$ once, and finishing at the response of the first run. In Section~\ref{sec:indempotence}, we show how to make any thunk involving \oread, \owrite{} and compare-and-modify (\cam) instructions into one that is idempotent with constant overhead.

% \paragraph{Achieving Idempotence.}
In this section we describe a simulation that converts a thunk involving \oread, \owrite{} and \cas{} instructions into one that is idempotent, and prove Theorem~\ref{theorem:idempotent}.    
We do this in a few steps. First, we present a construction with a few restrictions, and later, we show how to lift these restrictions. Namely, we begin by showing how to convert any thunk that (1) uses a constant amount of local memory, (2) does not make use of the return values of any \cas{} operation, and (3) we disallow concurrent \owrite{}s and \cas{}es to the same location inside the thunk.  To ease  readability, we call \cas{} operations that do not return any value \emph{compare-and-modify (\cam)} operations; thus, restriction (2) dictates that the thunk use \cam{} operations instead of \cas{es}.

After presenting the idempotence construction for the restricted setting, we show how to lift these restrictions.

%As the theorem states we do require a couple restrictions.  Firstly we require that a thunk have a constant amount of local memory, to which we refer as its \emph{registers} (these belong to the thunk independently of what process they run on).  All mutable state beyond the registers must be accessed via \oread, \owrite{} and \cam{} operations on memory locations.  
%We relax this condition in Section~\ref{sec:practicalities}, allowing for unbounded local memory, but with some restrictions on how the memory is used.  
%We also disallow concurrent \owrite{}s and \cam{}s to the same location.

\subsection{Idempotence Construction for Restricted Thunks}

In our simulation, each memory operation of the thunk is simulated by some number of other operations.  To help us discuss concurrent memory operations, we split each simulated memory operation into an invocation and response, and refer to the operations used to implement the simulation as \emph{primitive operations}.  A simulation is linearizable if, for each memory operation $op$ in the history of a simulation, the effect of $op$ happens between $op$'s invocation and its response.

% \begin{theorem}
% \label{theorem:idempotent}
% Any thunk with constant sized local memory and using only \oread{}, \owrite{} and \cam{} operations on shared memory can be simulated using \oread{}s, \owrite{}s and \cam{}s as primitive operations such that it is idempotent, and every simulated memory operation takes constant time (i.e., a constant number of primitive operations).  As long as there are no concurrent writes and CAMs on the same location, the simulation is linearizable.
%   \end{theorem}

  We base our simulation on two other operations, \emph{labeled load link} (\olll{}) and \emph{labeled store conditional} (\lsc{}).  An \olll{} takes a location and returns a ``label'' along with the value held at the memory location.  
An \lsc{} takes a destination location \texttt{loc}, a label \texttt{old}, and a new value \texttt{new}.  If \texttt{old} was the label returned by a \olll{} on \texttt{loc}, a later \lsc{} on \texttt{loc} will \emph{succeed} and write \texttt{new} to \texttt{loc} if and only if no successful \lsc{} to \texttt{loc} linearized between the \olll{} and \lsc{}.  If \texttt{old} was not read from \texttt{loc}, the behavior is undefined.  Note that the \olll{} and \lsc{} are similar to standard load-linked (LL) and store-conditional (SC) operations, but differ in that the \lsc{} need not be executed by the same process as the \olll{}.   Also here we are assuming the \lsc{} does not return whether it succeeded or not, unlike usually assumed for SC.
  
The \olll{} and \lsc{} operations can be implemented using standard techniques.  For example, an implementation can attach a counter to every memory location and when executing an \olll{}, return the counter as the label along with the value.  The \lsc{} can then be implemented by first checking if the counter is the same and getting the old value, and if the same executing a double word CAM conditionally replacing the old value and old-counter, with the new value and counter incremented by one.  This involves a double-word CAM (or CAS), but an implementation could avoid both a double-word CAS and an unbounded counter by instead using a level of indirection.  In this case the label is actually a pointer to the value, and the CAM just has to use the pointer for its old, and a new pointer to the new value for its new.  This requires some form of constant-time safe memory reclamation to ensure a pointer is only reused after no other process has access to it~\cite{blellochWei20}.

  \begin{figure}
\begin{lstlisting}
read(x) { return LLL(x).val;}

write(x, y) {
  lv = LLL(x);
  LSC(x, lv.label, y);}

CAM(x, old, new) {
  lv = LLL(x);
  if (new != old and lv.val == old) LSC(x , lv.label, new);}
\end{lstlisting}
    \caption{Simulating \oread, \owrite{} and \cam{} using \olll{} and \lsc{}.}
    \label{fig:labeled}
    \end{figure}

    Our simulation works in two stages. Firstly, we implement traditional \oread{}s, \owrite{}s and \cam{}s using \olll{} and \lsc{}, as shown in Figure~\ref{fig:labeled}.  Secondly we simulate an \lsc{} by adding a synchronization among processes.  The idea of the synchronization is to have all processes working on a thunk agree on the state of the thunk before making any updates (\lsc{}s).  We define a \emph{context} as the program counter and the current value of the registers for a thunk as it runs.  A context can be used to represent the original thunk since the captured arguments (or pointers to them) can be kept in the registers, and the program counter would point to the first instruction of the thunk.  We keep a copy of the context in memory, originally the initial thunk itself, and then periodically updated as the thunk proceeds.  We refer to this as the \emph{shared thunk}.  Each process running a thunk also keeps its own copy of the most recent context it read from memory, which we call the \emph{previous context}.  We run the thunk as normal, except that before every \lsc, we add a context update operation.  The context update does a multiword (adjacent words) CAM on the shared thunk with the expected value being the previous context, and the new value being the current context.  Note a multiword CAM can be implemented in constant time with a single-word CAM using indirection~\cite{blellochWei20}.   The purpose of the context update is to ensure that all runs of the thunk are in the same state before the \lsc{} (what is important is that all \lsc{} are applied with the same arguments). %\Naama{Whenever we do LCS you need a new capsule.}
We refer to the instructions between two context updates as a capsule.
The pseudocode is shown in Figure~\ref{fig:simulation}.   Without loss of generality we assume each context stored
to the \code{contextLocation} is unique.   If not, we can simply add a capsule number to the context to make it unique.

\begin{figure}
\begin{lstlisting}
previousContext;
sharedThunkLocation;

run():
  previousContext = Read(contextLocation)
  load previousContext into registers
  jump to program counter

runThunk(thunkPointer):
  sharedThunkLocation = thunkPointer
  run()

contextUpdate():
   copy registers into newContext
   CAM(sharedThunkLocation, previousContext, newContext)@\label{line:cam}@
   run()

simulatedLSC(loc, old, new):
  contextUpdate()
  LSC(loc, old, new)
\end{lstlisting}
  \caption{Simulating code containing \olll{} and \lsc{} so it is idempotent.   The \olll{} is unmodified and the \lsc{} uses
the \code{simulatedLSC}.}
  \label{fig:simulation}
\end{figure}

\begin{lemma}\label{lem:restrictedIdem}
	Any thunk using constant sized local memory and using only \oread{}, \owrite{} and \cam{} operations on shared memory can be simulated using \oread{}s, \owrite{}s and \cam{}s as primitive operations such that (1) it is idempotent, and  (2) every simulated memory operation takes constant time.  As long as there are no concurrent writes and CAMs on the same location, the simulation is linearizable.
\end{lemma}

\begin{proof}%[Proof of Theorem~\ref{theorem:idempotent}] 
  First we outline the correctness (linearizability) of the implementation of concurrent \oread{}s and \owrite{}s, and \oread{} and \cam{}s in terms of \olll{} and \lsc{}.  We do not allow concurrent \texttt{writes} and \texttt{CAM}s.  A \oread{} will always linearize at its \olll{}.  A \owrite{} will linearize on the \lsc{} if successful, and otherwise linearize immediately before the write that corresponds to the first successful \lsc{} after the \olll{}.  There must be one before the \owrite{}'s \lsc{} since it is not successful.  This gives the correct behavior when interleaved with \oread{}s since a \owrite{} will either appear to be immediately overwritten by a following successful \owrite{}, or will be properly written after its \lsc{}.  The \cam{} will linearize at the \olll{} if either of the conditions fail, and at the \lsc{} otherwise.   Again this gives the correct behavior when interleaved with \oread{}s.
 % to the same location, and indeed they would not be correct.  In particular a \texttt{CAM} could split the \olll{} and \lsc{} of a \texttt{write} causing it to fail on the \lsc{}, in the case that it would have caused the \texttt{CAM} to fail if linearized first---i.e., the \texttt{write} can be neither linearized before or after the \texttt{CAM}.  We now show that the \olll{}s and \lsc{}s are idempotent.  We note that \lsc{} is the only operation that updates shared memory.

  We consider the simulation based on \olll{}s and \lsc{}s.  We consider how the thunk progresses through its capsules, proving correctness by induction on $i$, where $i$ represents the $i$-th successful \cam{} of the context on Line~\ref{line:cam} by any process helping with the thunk.     In particular for $i$ we assume that the thunk is idempotent to that point, and
the context written is consistent with a single process running on the thunk to that point.   
We refer to the $i$-th context as $c_i$.   
At this point there might be processes that are still working on capsule $i$ (the one before the $i$-th successful \cam)
or even earlier capsules.
Firstly we want to show that no \lsc{}s from these earlier capsules can succeed.       We note that
if two calls are made to an \lsc{} with equal arguments, the second always fails.   This is because if the first \lsc{} succeeds
it falls between reading the label and the second causing the second to fail, and if the first fails some other \lsc{} fell beween
reading the label and it, which also falls between reading the label and the second, again causing the second to fail.
Now any \lsc{} from an earlier capsule $j \leq i$ will have read the same context as a capsule that has now completed its \lsc, and therefore had the same arguments for its \lsc{}, and will fail.

Secondly we take the first process running capsule $i+1$ that executes its \lsc{} step and add it to $H'$ (from Definition~\ref{def:idempotence}).   This is correct since it is the same instruction a single process running the thunk
would take.   Further \lsc{}s on step $i+1$ will fail since they have the same arguments.

Thirdly we want to ensure the next context written (at the end of capsule $i+1$) is correct.  This is because the first thing they all do is the \lsc{}.  Only the first can succeed, but immediately after the \lsc{} they are all in the same state.  This is where it is important that the \lsc{} does not return whether it was successful or not.  From this point until the end of the capsule the states might diverge since we are allowing for races with other procedures or thunks, but none of them are doing updates that are visible to each other, and at the end one will succeed on its \cam{} of a new context.  That one is a valid run of just a single process for that capsule since the \lsc, and we can add all its \olll{}s to $H'$.  We have thus shown our invariants hold after the $i+1$-th successful \cam{} of the context. 

Finally when the first process finishes (responds), all previous LCSs in $H'$ have been completed.
\end{proof}

\subsection{Removing the Restrictions}

Lemma~\ref{lem:restrictedIdem} shows that any thunk that satisfies some assumptions can be made idempotent. In this section, we show that these assumptions are in fact not restricting; we can systematically convert any thunk that does not satisfy them into one that does. This will result in the final general result of Theorem~\ref{theorem:idempotent}.

We first handle the restriction on constant private memory. If a thunk uses more than a constant amount of private memory, we move its private memory into a shared memory region that is allocated specifcally for this thunk. It must then use shared reads and writes when accessing this memory instead of private ones. We make this change before applying the construction discussed in the previous subsection, and therefore, any reads and writes into this memory will be treated as shared ones and replaces with LLLs and LSCs as described in the construction. This adds constant overhead, and allows a thunk to use only shared memory.

Next, we note that Aghazadeh et al~\cite{aghazadeh2014making} present a construction that removes races between \cas{} and write operations by replacing the memory on which such races happens with a \emph{writable CAS (wCAS)} object. This object is implemented in constant step complexity per operation using $n^2$ \cas{} primitive objects where $n$ is the number of processes in the system. Ben-David et al~\cite{ben2019delay} later presented a more space-efficient version. The idea of the construction is to use a level of indirection to direct \cas{} and writes on the same object to different memory locations. At a high level, the object stores a pointer to the memory location in which its value its stored. Reads and \cas{} operations are executed on the value itself, after following the pointer to it. Write operations instead allocate a new memory location with the value, and then execute a \cas{}  to swing the pointer to it. In this way, write and CAS operations that would have races on the same memory location no longer race. We can therefore use this construction to convert any thunk with write-CAS races into one in which writes and \cas{es} do not race. The correctness of this construction (its linearizability and step complexity) is proven in~\cite{aghazadeh2014making}.

Finally, we rely on another construction by Ben-David et al.~\cite{ben2019delay} to show that any \cas{} can be implemented using only \cam{s}. That is, we show how to store the return value of a \cas{} separately from the \cas{} itself, to allow it to be recovered after executing the operation if an algorithm requires it. This construction uses only a constant number of \cam{} operations (i.e., does not require the return values of its primitive \cas{} operations). For this, we use the \emph{recoverable CAS} construction presented in~\cite{ben2019delay}. In their construction, they implement a CAS object with an extra `recover' operation that can be called to recover the return value of the last \cas{} operation executed on the object. Their implemenation of this object uses a constant number of \cas{} primitive operations, and does not use the return value of any of them. We therefore use this construction directly to replace a \cas{} operation in a thunk by a \cam{} implementation as follows: call the \cas{} operation of the recoverable CAS object, discarding its return value, and then call the recover operation of that object.  In this way, any thunk that makes use of its \cas{} operations' return value can be rewritten as a thunk with only \cam{s}. The correctness of this conversion is proven in~\cite{ben2019delay}.

%Finally, we tackle the restriction on the constant sized private memory of the thunk. Note that this requirement is needed to ensure that each context takes a constant time to update. To maintain a larger amount of private memory, a thunk can keep its private memory on a shared memory region specifically allocated to it. The context update then works a bit differently, as follows. Let $C$ be the set of `private' memory locations that the thunk changes in a given capsule (between two consecutive context updates). Instead of directly applying the changes, we aggregate these in a buffer, where, for each value, we keep the location to be updated, and the old and new values. We include this buffer in the new context. After updating the context and before executing any other implemented operations of the original thunk, we apply these changes to the memory using \cas. In this way, we keep the context update time constant, but allow the thunk to use an arbitrary amount of local memory. A process attempting to execute the thunk using an outdated context will fail to update the values of $C$ in the thunk's private memory region, assuming the ABA problem does not occur. We can avoid the ABA problem by attaching counters to each memory location in the thunk's private memory region. \Naama{W.l.o.g. constant memory -- if non constant, move some of it to shared, use shared writes, resplit into capsules with this.}
%with the location to be updattedThe context then contains, for each `private' memory location updated since the last context update, the old and new value. After the context is updated, the 

In this way, we have removed all restrictions imposed by Lemma~\ref{lem:restrictedIdem}, and therefore Theorem~\ref{theorem:idempotent} holds.



  \subsection{Practical Considerations}
  \label{sec:practicalities}
  
  Although the simulation is not particularly cumbersome, there is still overhead involved in the multiword CAM used in \texttt{contextUpdate}.  Here we point out that there are several ways to reduce the number of \texttt{contextUpdate}s (i.e. capsules).  Importantly, any number of simulated \lsc{}s on distinct locations can run in the same capsule, as long as they are all at the start of the capsule, i.e., immediately after the \texttt{contextUpdate} and before any \olll{}s.  Also, any static data need not be written to the shared context.  Many potential uses of our fair locks would require at most two capsules with only one or two registers saved across the boundary.  This would be the case, for example, in locked operations on a stack or queue.

% With regards to only allowing a constant number of local memory locations (registers), this can be loosened in the following way without effecting any of the bounds.  In addition to the constant number of registers, each thunk can have unbounded number of of write-once local memory locations.  In particular a write-once memory location can only be written once by the thunk, and can only be read by the thunk after writing.     These
  


==> lock-proof.tex <==
\section{Analysis of Lock Algorithm}\label{sec:single-lock-proof}

To analyze the algorithm, we begin with a few definitions, including how we define the amount of contention that a given \op{} experiences.



We associate each \op{} to grab the lock with the priority that it chooses at the beginning of its execution. 
We say that an \op{} \emph{succeeds} if its returns \texttt{true}, and that it \emph{fails} otherwise. 
%\Naama{Need to prove that an \op{} succeeds iff its priority gets written into \live{} before the end of its execution.}

Note that the only CAS that is ever executed on the \docket{} is on line~\ref{line:tryClear}, and uses $NULL$ as the new value. That is, its purpose is to clear the \docket{}'s previous contents. We therefore sometimes refer to a CAS on the \docket{} as a \emph{\tryclear{}}.
% The CASes on line~\ref{line:tryClear1} and on line~\ref{line:tryClear2} are called the \emph{\tryclear{}}.

%\Naama{Should define `attempt'. A call to the \texttt{lock} function?}

\begin{definition}
	An \op{} $op$'s \emph{\wwmtime{}} is the time at which it executes its write-with-min.
\end{definition}

\begin{definition}
	A read of the \docket{} on line~\ref{line:rdlive} that provides the new value for a successful CAS on line~\ref{line:liveCAS} is called a \emph{\critread{}}.
\end{definition}

We now define special instructions that we say are \emph{associated} with a given \op{} executed by some process $q$. These instructions happen during the \op's execution interval, but are not necessarily executed by $q$ itself. As we will see in the proof, these particular instructions and their timing with respect to the progress of other concurrent \op{s} will be crucial in determining the success or failure of the \op.

\begin{definition}
	The first \critread{} after an \op{} $op$'s \wwmtime{} is called $op$'s \emph{\firstcritread{}}. 
\end{definition}

\begin{definition}
	The successful CAS on the \live{} on line~\ref{line:liveCAS} that got its new value from $op$'s \firstcritread{} is called $op$'s \emph{\firstsuccCAS{}}.
\end{definition}

\begin{definition}
	The first CAS on the \docket{} whose old value was read from \live{} after $op$'s \firstsuccCAS{} is called $op$'s \emph{\assocClear{}}.
\end{definition}

We now have enough terminology to start analyzing the execution of an \op, and to define the amount of contention that it experiences. For this purpose, we consider sub-intervals  of an \op's execution.

\begin{definition}
	An \op{} $op$'s \emph{\activeInt{}} is the interval between its \wwmtime{} and its \assocClear{}.
\end{definition}

\begin{definition}
	An \op{} $op$'s \emph{\dangerInt{}} is the interval between its \wwmtime{} and its \firstcritread{}.
\end{definition}


\paragraph{Safety.}

We now show that  Algorithm~\ref{alg:single-lock} is correct. That is, we show that it ensures the following safety conditions:
\begin{itemize}
	\item At most one process holds the lock at any point in time
	\item A process's \op{} is successful if and only if its thunk gets executed to completion before the end of its \op{}
\end{itemize}
%In the next subsection, we prove that it also satisfies our desired fairness guarantees.

We begin the proof with a couple of useful lemmas.
For convenience, we say that `an \op{} $op$ is written in \live{}' if $op$'s priority is written in \live{} while $op$'s descriptor was in the corresponding slot of the announcement array.  %\Naama{Rephrase this to match putting descriptor directly into live slot.}

\begin{lemma}\label{lem:CasInLoop}
An \op's \firstsuccCAS{} must happen before the end of the execution of its own for loop.
\end{lemma}

\begin{proof}
Consider an \op{} $op$ by process $q$. First note that if one of $op$'s CASes on \live{} was successful, then that CAS was either itself $op$'s \firstsuccCAS, or it happened after $op$'s \firstsuccCAS. In either case, the lemma holds.

We now assume that both \Naama{says `both', even though the compete() loop had 3 iterations.} CASes on \live{} executed by $op$ fail. Note that for any process to execute a successful CAS on \live, it must read \live, and then read the \docket{} before executing the CAS. For $op$ to fail its first CAS, another successful CAS, $c_1$, must have happened between when $op$ first read \live{} and when it executed this CAS. In particular, $c_1$ happened after $op$'s \wwmtime. For $op$ to fail its second CAS, yet another successful CAS, $c_2$, on \live{} must have happened before $op$ executed its second CAS on \live. Let $p$ be the process that executed $c_2$. For $c_2$ to succeed, $p$ must have read \live{} after $c_1$ occurred. In particular, this means that $p$ also read the \docket{} after $c_1$. Recall that $c_1$ happened after $op$'s \wwmtime. Thus, $c_2$ is a successful CAS that occurred after $op$'s \wwmtime, and before the end of $op$'s for loop. That is, $c_2$ is either itself \firstsuccCAS{} or happened after $op$'s \firstsuccCAS. In either case, the lemma holds.
\end{proof}

\begin{lemma}\label{lem:LiveMeansDone}
	Any \op{} that gets written into \live{} gets its descriptor executed and its done flag set to true before being removed from \live.
\end{lemma}

\begin{proof}
Assume by contradiction that there is some \op{} $op$ that was written in \live{} but was overwritten before getting its descriptor executed to completion. Let $q$ be the process that overwrote $op$'s priority in \live. Note that \live{} only ever gets updated with a CAS whose old value was read from \live{} by the process that execute the CAS. For $q$'s CAS to have been successful, it must have read $op$'s priority  from \live{}. Note also that between every read of \live{} and the following CAS into \live{} by the same process, \texttt{help()} is called on the \op{} whose priority was read. Therefore $q$ must have called \texttt{help()} with $op$'s priority. Since \texttt{help()} executes the descriptor pointed at by its argument to completion before returning, $op$'s descriptor must therefore have been executed and its done flag set  to true before $q$ executed the CAS that removed $op$'s priority from \live. Contradiction.
%\Naama{mention reason why $op$'s descriptor must remain in the same slot of the announcement array the entire time?}
\end{proof}

\begin{claim}\label{clm:safe}
	An \op{} succeeds if and only if its priority gets written into \live{} and its descriptor is executed.
\end{claim}

\begin{proof}
It is easy to see that if an \op{} returned `success', then its priority must have been written into \live. To see this, note that \texttt{help}($\ell$) is the only place in which \texttt{announce[$\ell$].done} gets updated and in which any descriptor gets executed, and that \texttt{announce[$\ell$].done} is initialized to false for all slots of the array. Note also that \texttt{help}($\ell$) is only ever called with a value $\ell$ that was read from \live. Thus, the \texttt{done} field can't be set to true for any slot in the announcement array unless the corresponding \op{}'s priority was written into \live{} and its descriptor was executed.

We now show that if an \op{} $op$ by process $q$ returns `failure', then at no point was it written in \live. 
%We do this by showing that $op$ can only be written into \live{} before the end of its own for loop, and that if it does, its \texttt{done} flag gets set to true before $q$ reads that flag. 
Note that an \op{} $op$ gets written into \live{} if and only if its \firstsuccCAS{} has $op$'s priority as its new value; this is because its priority does not get re-written into the \docket{} during its execution. By Lemma~\ref{lem:CasInLoop}, $op$'s \firstsuccCAS{} is during its own for loop. Therefore, $op$ can only ever get written into \live{} by the end of its own for loop. Furthermore, by Lemma~\ref{lem:LiveMeansDone}, if $op$ did get written into \live, then its \texttt{done} flag gets set to true before being overwritten. To complete the proof, note that if $op$ does not get overwritten in \live{} before the end of its execution, then $q$ itself executes \texttt{help()} with $op$'s priority before completing the \op, thereby ensuring that its \texttt{done} flag gets set to true and that it returns `success'.
\end{proof}

Note that since we define a process $q$ to be `holding the lock' at a given time $t$ if $q$'s priority is the value in \live{} at  time $t$, by definition there is only one process holding the lock at any given time. This, combined with Claim~\ref{clm:safe}, completes the safety argument for Algorithm~\ref{alg:single-lock}.
We now shift our focus to proving the efficiency and fairness guarantees.

\paragraph{Efficiency and Fairness.}

Intuitively, to capture the fairness of the algorithm, we show that an \op{} $op$ will fail if and only if some other \op{} with a higher priority overlaps with $op$'s \dangerInt{}. Furthermore, we show that the set of priorities that a given \op{} $op$ competes against is always uniform and i.i.d., and its size is at most twice the point contention that $op$ experiences. Therefore, if $op$ found an announcement slot, $op$'s probability of success is simply the probability that its priority is the highest of at most $2\kappa$ uniform, independent, and identically distributed random variables (i.e. $\geq \frac{1}{2\kappa}$), where $\kappa$ is the point contention $op$ experiences in its execution.

%At a first glance, it may look like a scheduler could potentially reschedule a descriptor whose \op{} failed to compete over and over again against the same \op{} against which it lost. This would violate the guarantee that each \op's success probability depends only on the point contention during its execution, and not on past failures. Furthermore

%we show that it is impossible for a descriptor whose \op{} failed to compete against the same \op{s} when it retries. More specifically,
%
%\Naama{Remove the game argument. Leaving for now to reread, but should be able to kick out completely. Seems only helpful when we are trying to argue about a stronger adversary.}
%To prove our claims that each attempt has a \emph{fair chance} at acquiring the lock, we must argue about what power the adversarial scheduler has. To do so in a clean manner and decouple arguments about concurrency from arguments about the probability of success, we define a game between players and an adversary, and split the analysis in two steps; first we show  that Algorithm~\ref{alg:single-lock} adheres to the rules of the game, and then we show that in this game, the adversary cannot force each player to win with probability less than $1/t+1$ where $t$ is the number of other players the adversary introduced into the game.
%
%The game consists of two queues: the \emph{dangerous} queue and the \emph{safe} queue. It proceeds in rounds, in which the adversary makes the following decisions: (1) it may enqueue some set of new participants into the dangerous queue, (2) it may choose some prefix \Naama{get rid of the word prefix; it's confusing} of the dangerous queue to move to the safe queue \Naama{Actually, i think it has to be all of the danger queue or none of it}, and (3) it may choose some prefix of the safe queue to remove from the game. We refer to all participants in either queue collectively at some time $t$ the \emph{active} set at $t$. When a participant $p$ enters the dangerous queue (becomes active), it does so with a hidden priority. When it is removed from the safe queue, the priority  is revealed to the adversary. If, during the time that $p$ was in the dangerous queue, there was some other active participant $p'$ with a priority higher than $p$'s, then $p$ loses. Otherwise, $p$ wins. \Naama{Is there a cleaner way to describe this game?}
%
%\Naama{Another description of the game: two rooms/zones with FIFO enter-exit order. The first room everyone leaves at once (although maybe that just makes it more confusing). }
%
%\Naama{Maybe we can simplify the game because we are assuming a completely oblivious adversary.}
%
%\paragraph{Relevance of the game.} At first glance, it might not be obvious why this game characterizes the behavior of the lock algorithm. Intuitively, we show that an attempt $op$'s \emph{\dangerInt} corresponds to the time it spends in the dangerous queue in the game, in that  $op$ will fail if and only if during that time, some other ongoing attempt has a higher priority than $op$. Furthermore, we argue that the priorities of the attempts have no affect on the number of steps that they take. This means that an oblivious scheduler completely determines the set of descriptors that will be active during a given attempt's \dangerInt. Thus, since the oblivious adversary makes this decision in advance, before the priorities are chosen, the priorities a given attempt competes with are independent and uniformly distributed.
%%we argue that the adversary cannot gain any information about an attempt's priority until after that attempt has been written into \live, at which point (as we've shown in Section~\ref{sec:lockSafety}), it is guaranteed to succeed.

We say that a successful CAS on \live{}, along with the read of \live{} by the same process that immediately preceeded it, are together a \emph{Read-SCAS pair}.
	
\begin{lemma}\label{lem:SCASpairs}
 Read-SCAS pairs do not overlap. %\Naama{This assumes we have no ABA problem. Should be fine if we ensure priorities aren't repeated while someone is holding them, and that the priority is cleared before you stop holding it. Should be easy using the array of priorities/descriptor slots.}
\end{lemma}

\begin{proof}
	Assume by contradiction that 2 Read-SCAS pairs, $s_1$ and $s_2$ overlap in some execution. Denote by $s_1.r$ and $s_2.r$ the reads of $s_1$ and $s_2$ respectively, and denote by $s_1.c$ and $s_2.c$ the successful CASes of $s_1$ and $s_2$ respectively. Assume without loss of generality that $s_1.c$ happened before $s_2.c$. Since the intervals are overlapping, $s_2.r$ must have happened before $s_1.c$. In particular, $s_2.r$ read an earlier value than the one that $s_1.c$ successfully wrote in \live{}.  However, since values in \live{} do not repeat, and the value read by $s_2.r$ is used as the old value of $s_2.c$, $s_2.c$ must have failed, contradicting the assumption that $s_2$ is a Read-SCAS pair.
\end{proof}

\begin{claim}\label{clm:cleared}
	An \op{} $op$'s descriptor cannot be in the \docket{} after $op$'s \assocClear{}.
\end{claim}

\begin{proof}
	Clearly, if the clear was successful, $op$'s descriptor has been cleared from the \docket{}. 
	%\Naama{Unless the priority  is being reused by another \op{} now. Need to change lemma statement to only apply while $op$ is still active.} 
	So, assume the CAS of $op$'s \assocClear{} failed.
	Note that by the definition of $op$'s \assocClear{}, its old value was read from \live{} after $op$'s \firstsuccCAS{}. Note also that by the definition of an \op{}'s \firstsuccCAS{} and its \wwmtime{}, the new value written into \live{} by $op$'s \firstsuccCAS{} was read from the \docket{} after $op$'s \wwmtime{}. Furthermore, the \live{} field is only ever updated with new values that were read from the \docket{} and, by Lemma~\ref{lem:SCASpairs}, cannot be updated to a value that was read from the \docket{} earlier than the value it already had. For the clear to fail, the \docket{} must have been updated since the \critread{} of the most recent successful CAS on \live{}, and in particular, since the \firstcritread{} of $op$.
	
	Thus, if the \assocClear{} of $op$ failed, the \docket{} must have been updated since $op$'s \firstcritread{}, which was after $op$'s \wwmtime{}. Thus, the value it announced can no longer be in the \docket{}.
\end{proof}

\begin{definition}\label{def:threaten}
	An \op{} $op_1$ \emph{threatens} \op{} $op_2$ if $op_1$'s \activeInt{} overlaps with $op_2$'s \dangerInt{}.
\end{definition}

%\begin{definition}
%	An \op{} $op_1$ \emph{blames} \op{} $op_2$ if $op_2$'s priority is in the \docket{} immediately after $op_1$'s \wwmtime{}, or $op_2$'s priority is returned by $op_1$'s \firstcritread{}.
%\end{definition}

\begin{definition}\label{def:blame}
	An \op{} $op_1$ \emph{blames} \op{} $op_2$ if $op_2$'s descriptor is returned by $op_1$'s \firstcritread{}.
\end{definition}

\begin{claim}\label{clm:blame}
	If \op{} $op_1$ blames \op{} $op_2$ then $op_2$ threatens $op_1$ and $op_2$'s priority is higher than $op_1$'s.
\end{claim}

\begin{proof}
	This claim derives directly from the definitions of blame and threat. 
	Let $t$ be the time at which $op_1$'s \firstcritread{} is executed.
	For $op_1$ to blame $op_2$, $op_2$'s descriptor must be written in \texttt{docket} at $t$. Note that if $op_2$ doesn't threaten $op_1$, then either it ended before $op_1$'s interval began, or it started after $op_1$'s \dangerInt{} ended. In the former case, by Claim~\ref{clm:cleared}, $op_2$'s descriptor cannot be in the docket. In the latter case, recall that $op_1$'s \dangerInt{} is defined to end at $t$. Thus, it is impossible for $op_2$'s descriptor to be in the docket already, if it didn't already start its interval. Therefore, it is clear that for $op_1$ to blame $op_2$, $op_2$ must threaten $op_1$. 
	
	Furthermore, note that $t$ must be after both \op{s} executed their  \wwm{}. If $op_2$'s descriptor is written in the docket at time $t$, then its \assocClear{} hasn't happened yet. Therefore, at time $t$, both \op{s} have executed their  \wwm{} but not yet cleared it. By the correctness of  \wwm{}, if $op_2$'s descriptor is written in \texttt{docket} at that time, then $op_2$'s priority is higher.
\end{proof}

\begin{claim}\label{clm:early-end}
	If an \op{} $op_1$ threatens an \op{} $op_2$ then $op_1$'s \activeInt{} ends at the same time as or earlier than $op_2$'s interval.
\end{claim}

\begin{proof}
	Note that by the definitions of \firstcritread, \firstsuccCAS, and \assocClear, if two \op{s} have the same \firstcritread, then they have the same \firstsuccCAS{} and \assocClear{} as well. Furthermore, if an \op{} $op_1$'s \firstcritread{} is before another \op{} $op_2$'s \firstcritread, then $op_1$'s \firstsuccCAS{} and \assocClear{} must be either before those of $op_2$ or at the same time as those of $op_2$. 
	
	Let $op_1$'s \firstcritread{} be at time $t_2$, and let $op_2$'s \firstcritread{} be at time $t_2$.
	Furthermore note that by definition, $op_1$ threatens $op_2$ if and only if $t_1 \leq t_2$. Therefore, as argued above, $op_1$'s \assocClear{} must also be earlier or at the same time as $op_2$'s \assocClear.
\end{proof}

\begin{claim}\label{clm:point-contention}
	The number of \op{s} that threaten a given \op{} $op$ is at most $2\kappa$, where $\kappa$ is $op$'s point contention.
\end{claim}

\begin{proof}
	Let $t$ be the time at which $op$ executed its  \wwm{}(thus starting its \dangerInt), and let $t'$ be the time of $op$'s \firstcritread{} (thus, the time at which $op$'s \dangerInt{} ends). Note that the number of \op{s} that threatened $op$ is at most $\kappa(t) + \kappa(t') + \vert Fast \vert$, where $Fast$ is the set of \op{s} that started their conflict interval after $t$ and finished it before $t'$. However, note that any \op{} in $Fast$ must have been theatened by $op$. Therefore, by Claim~\ref{clm:early-end}, any  such \op{} cannot have finished its conflict interval before $op$. Therefore, $\vert Fast \vert = 0$.
	Thus, the number of \op{s} that threaten $op$ is at most  $\kappa(t) + \kappa(t') \leq 2\kappa$.
\end{proof}

%\begin{claim}
%	If help($\ell$) gets called with $\ell$ being $op$'s priority, $op$'s \assocClear{} must have happened by the time immediately after line~\ref{line:tryClear} is executed during this call to help($\ell$). 
%	%its \assocClear{} must have happened before the first call to help with $\ell$.
%\end{claim}


%\begin{claim}
%	As long as no \op{} reached the end of its interval, the scheduler gained no information on any \op{}'s priorities.
%\end{claim}
%
%\begin{claim}
%	When an \op{} $op$ reaches the end of its interval, the scheduler does not know whether any \op{} blamed it.
%	\Naama{Consider two \op{}s $op_1$ and $op_2$ such that $op_1$ threatens $op_2$. The scheduler does not know whether $op_2$ blamed $op_1$ until after both \op{}s' intervals end.}
%\end{claim}
%
%\begin{claim}
%	When the scheduler chooses to have $op_1$ threaten $op_2$, it has no information on the priorities of either \op{}.
%\end{claim}

%\Naama{Old stuff below.}
%
%Thus, we can view Read-SCAS pairs as sequential with respect to each other. We use these Read-SCAS pairs to define the contention interval of each \op{}. Intuitively, the interval of each \op{} is defined by the Read-SCAS pairs between which its write-with-min (WWM) instruction falls.
%
%\begin{definition}
%	Consider an \op{} $op$ that executes its  \wwm{}at time $t$. $op$'s \emph{interval} is defined as the interval of time from 
%	its own \wwm{}
%	%the latest TryClear CAS that happened before $t$,
%	%the latest special read that happened before $t$, 
%	until the end of the \tryclear{} associated with the following Read-SCAS pair.
%	$op$'s \emph{InDanger} interval is the prefix of its interval that is before the special read of the final Read-SCAS pair in its interval.
%	%An \op{}'s interval is partitioned into two parts; the \emph{InDanger} part is from the beginning of the interval until the special read of the second Read-SCAS pair in the interval, and the \emph{CauseDanger} part is the rest of the interval. \Naama{Now with a \tryclear{} executed immediately after each special read, we can probably say the interval starts at the most recent \tryclear{}, rather than the most recent special read. If that's true, that should solve the issue of contending with people who finished long before you started...}
%\end{definition}
%
%We say that $op_1$ \emph{contends with} $op_2$ if $op_1$'s In\dangerInt{} overlaps with $op_2$'s interval. Note that by this definition, contending is an asymmetric relationship. \Naama{make definition for contend. Also make it sound more asymmetric.}
%%two \op{}s \emph{contend} if their intervals overlap. \Naama{To be ammended for the appropriate parts of the interval.}
%
%\begin{theorem}
%	An \op{} $op$ whose In\dangerInt{} overlaps with the intervals of $c$ other \op{}s has a probability of at least $1/c$ of success.
%\end{theorem}
%
%The key to showing this theorem is to show that if an \op{} $op_1$ does not contend with another \op{} $op_2$, then $op_2$ cannot make $op_1$ fail. 
%%
%%We prove this theorem in two parts; first, we show that if two \op{}s $op_1$ and $op_2$ do not contend, then they cannot make each other fail. 
%Thus, only \op{}s that a given \op{} $op$ contends with could lower its probability of success. 
%Furthermore, an adversary that only gets access to the execution so far cannot bias the distribution of priorities that an \op{} contends with.
%%In the second part of the proof, we show that the distribution of priorities of \op{}s that contend with $op$ is uniform on the entire range of probabilities. That is, the specific execution does not affect the priorities of contending \op{}s, and thus cannot skew the probability of success.
%
%To begin, we define a \emph{blame} relationship among \op{}s. Recall that an \op{} fails if and only if its priority doesn't get written into \live{}. This could happen either because its priority never got written into the \docket{} in the first place (it lost on its \wwm{}), or its priority was overwritten before the next special read. We thus define the blame relationship to capture all \op{}s that could potentially prevent a given \op{} from succeeding. \op{} $op_1$ \emph{blames} \op{} $op_2$ if (1) $op_2$'s priority was the value in the docket at the time that $op_1$ executed its \wwm{}, or if (2) $op_2$'s  \wwm{}was after $op_1$'s  \wwm{}and before the next special read. %\Naama{Relationship to In\dangerInt{} of $op_1$?}
%
%\begin{lemma}\label{lem:movetolive}
%	After any \op{} $op$ exits the for-loop, the value in \live{} is a priority that was written into \docket{} at a time greater than or equal to the time of $op$'s \wwm{}.
%\end{lemma}
%
%Lemma~\ref{lem:movetolive} shows that the interval of each \op{} ends while that \op{} is still active. That is, an \op{} does not depend on any other active process to complete its own interval. In particular, the only reason for an \op{} $op$ to fail is if someone who started after $op$ grabbed the lock. 
%%In this sense, the algorithm is \emph{lock-free}. 
%\Naama{The lemma is just for showing that the interval we defined is contained within the \op{}'s active time interval. That's important because we don't want an \op{} `succeeding' (i.e., being written into the \live{} slot) after that \op{} has already terminated with failure. So, could relate to showing that getting written into \live{} is equivalent to returning true. }
%%has two purposes: for showing that the interval we defined is actually contained within the \op{}'s active time interval (is this necessary?), and for showing that conflicting with a lower priority than you cannot make you fail.} %lock-freedom, I think. Not really lock freedom... something else.}
%
%\begin{lemma}\label{lem:tryclear}
%	The value of the \docket{} must change during any \op{}'s interval, after that \op{}'s \wwm{}.
%	\Naama{could be rephrased to be more precise.}
%	%	Consider an \op{} $op$. By the time $op$'s interval ends, the 
%\end{lemma}
%
%\begin{proof}
%	Recall that an \op{}'s interval ends with a TryClear CAS. Note that if that TryClear CAS succeeded, then it overwrote the value in the \docket{}, and thus the claim holds. We therefore focus on the case in which the TryClear at the end of the \op{}'s interval failed. In the TryClear failed, then some other process has changed the docket since it contained the value $\ell$ that the TryClear read from \live{}. Recall that $\ell$ was read from \live{} after the critical SCAS in the \op{}'s interval. 
%	\Naama{To be continued. Just need to show that the \op{}'s  \wwm{}happened before the value currently in \live{} was written, so if the docket is different from the value in \live{}, then it is more up-to-date than the \op{}'s \wwm{}. Should be easy but I don't quite see it.}
%\end{proof}
%
%\begin{lemma}\label{lem:blame}
%	If \op{} $op_1$ blames \op{} $op_2$, then $op_2$'s interval overlaps with $op_1$'s In\dangerInt{}.
%\end{lemma}
%
%\begin{proof}
%	Clearly, if $op_1$ blames $op_2$ because of reason (2), then $op_2$'s interval overlaps with $op_1$'s In\dangerInt{}.
%	By Lemma~\ref{lem:tryclear}, if $op_2$'s value is still in the \docket{} at some time $t$, then $op_2$'s interval has not ended by that time. In particular, if $op_2$'s value was in the \docket{} at the time $op_1$ executed its \wwm{}, $op_2$'s interval overlaps with $op_1$'s In\dangerInt{}. Thus the claim also holds if the blame is due to reason~(1).
%%	Assume by contradiction that $op_1$ blames $op_2$, but $op_2$'s interval doesn't overlap with $op_1$'s In\dangerInt{}. Then note that $op_2$ could not be blamed for reason (2). That is, by the definition of the \op{} interval and In\dangerInt{}, since $op_2$'s interval doesn't overlap with  $op_1$'s In\dangerInt{}, it must be the case that $op_2$'s  \wwm{}happened after the special read immediately after $op_1$'s \wwm{}, or that $op_2$'s interval was complete before $op_1$'s  \wwm{}was executed. 
%%Thus, it must be the case that $op_2$ is blamed by $op_1$ because its priority was in the docket at the time that $op_1$ executed its \wwm{}. However, recall that $op_2$'s interval ends with a \tryclear{}. Note that immediately after the \tryclear{} is executed, the docket must contain a value other than $op_2$'s value; either the \tryclear{} succeeded, thus clearing the docket, or it failed, meaning that some other process has changed the docket since $op_2$ last read live. By Lemma~\ref{lem:movetolive}, the value $op_2$ read in \live{} is at least as up to date as $op_2$'s \wwm{}, and thus if it failed in its \tryclear{}, the docket no longer contains $op_2$'s value.
%\end{proof}
%
%
%
%\begin{corollary}
%	If \op{} $op_1$ executed by process $p_1$ blames some \op{} $op_2$, then $p_1$'s next \op{} cannot blame $op_2$.
%\end{corollary}
%
%\begin{proof}
%	\Naama{has to do with $op_1$'s \tryclear{} happening before the end of its interval, and cutting off $op_2$'s interval if $op_2$ was advanced enough. We should only care about this `advanced enough' case because otherwise $op_2$ wouldn't have overlapped $op_1$'s \emph{InDanger} interval (if all goes well).}
%\end{proof}
%
%

%\begin{lemma}
%	An \op{} $op$ can't fail directly because of an \op{} whose interval doesn't overlap with the In\dangerInt{} of $op$. \Naama{Should define what we mean by fail directly. Other sublemmas are in the notes.}
%\end{lemma}

%\begin{lemma}
%	An \op{} $op$'s probability of succeeding is at least $1/c$ where $c$ is the number of \op{}s its In\dangerInt{} overlaps with.
%\end{lemma}
%
%\begin{proof}
%	Recall that the priorities of all \op{}s are drawn independently and uniformly randomly from the same interval. Let $X_i ~ Uni()$ be the i.i.d. variable representing the priority of the $i$'th \op{} in the history, where we order \op{}s by the time at which they execute their \wwm{}. Note that if $X_i \leq X_j$ for all $j$ that $i$ can blame, then $i$ succeeds. \Naama{Need to show that this is true. i.e. A lower priority \op{} that conflicts with you cannot make you fail. For this, we might need Lemma~\ref{lem:movetolive}, or we could argue this purely from the definition of your interval including a complete read-SCAS pair.} Furthermore, since the adversary only has access to the execution trace, it cannot gain information about the priorities of \op{}s, and thus cannot affect their distribution. \Naama{Formalize this?}
%	%We denote by $dangerInt(i)$ the In\dangerInt{} of \op{} $i$, and by $int(i)$ the entire interval of $i$. Recall from Lemma~\ref{lem:blame} that $i$ can only blame \op{}s whose intervals overlap with $dangerInt(i)$. So, we can bound $i$'s probability of success as follows.
%	\[ P[success_i] \geq P[\forall j \in BlameSet(i): X_i \leq X_j ]  = 1/c	\]
%	%\[ P[success_i] \geq P[X_i \leq X_j \forall j > i, j \in dangerInt(i) \wedge X_i \leq min_{j:i \in int(j)} X_j]  = 1/c	\]
%%	\Naama{Could have better notation. Need to mention that the adversary can't affect anything.}
%\end{proof}

%\Naama{Is it overlapping with the entire interval or just the Cause\dangerInt{} of the others? How can we get rid of the fact that with this interval definition, you always contend, even if you are completely alone?}

%Once we show this lemma, assuming an oblivious adversary should yield the result, since the oblivious adversary cannot see the values, and our conflicts are not affected by whether some \op{} succeeded or failed. \Naama{Another factor we might need to worry about: need to show that the frequency of Read-SCAS pairs isnt' affected by the number of \wwm{}s that have happened (i.e. that Read-SCAS pairs are also independent of the priorities seen).}
%\Naama{Need to show that length of interval gives no indication of how good someone's priority was. This should be easy because regardless of priority you execute the same instructions and end at the same time... kind of hand-wavy though.}


%\paragraph{Analyzing the game.}
%
%\Naama{We  had two analyses, neither one exactly what we wanted:
%\begin{enumerate}
%	\item Oblivious adversary: if the adversary only receives the step number as an input to the scheduling function, then it is oblivious. In this case, we can show that no information about the priorities is revealed to it even after an \op{} ends. So the game changes in that the adversary doesn't find out the priority when it removes them from the safe queue. So, the only thing the adversary can do is inflate the number of threateners you face, but this can't affect  the distribution of their priorities. Therefore, your chance of success is the same as being the min out of $t+1$ samples of a uniform distribution; $1/(t+1)$.
%	
%	\item No worse than the worst case contention: Let's say there is some maximum $M$ for the number of threateners the adversary is allowed to introduce. So, the only decision an adversary can make is whether to increase the number of threateners you face, to a maximum of $M$. When it chooses to introduce more threateners, it doesn't know their priority, so they are uniformly distributed. Can't get worse than $1/M$ chance of success.
%\end{enumerate}
%
%For the latter option, we thought that when we argue about using this within a larger program that has many such locks, we can give quite a good bound on the worst case any of them might face at any time (probably assuming some reasonable distribution of the operations across a data structure, i.e. they don't all aim to grab the same lock). Without any such assumptions, we can bound the number of threateners anyone can have by $2P-1$.
%
%One more option we considered is trying to prove that given a specific adversary (scheduling function) the average/amortized contention across all executions for each process's attempts is $c/(t+1)$ for some constant $c$. Or, even better, that even without amortizing across the possible executions, we are just a constant off from optimal. However, we didn't have that analysis complete.}


==> lockProofs.tex <==
\section{Lock Algorithm Safety Proof}\label{sec:lockProofs}

%\guy{[Reviewer says: ``I think, technically, you need something stronger:  that all priorities (of all processes involved) be mutually independent'']}

%\subsection{Safety Proof}

\begin{lemma}\label{lem:stableStatus}
	A  \descriptor{}'s status can change at most once during its execution.
\end{lemma}

\begin{proof}
	Note that the status of a \descriptor{} is only changed in the \code{eliminate} and \code{decide} functions, both of which use a CAS with an old value of \code{active} and if successful, change the status away from \code{active}.
\end{proof}

\begin{lemma}\label{lem:doneStatus}
	After a call to \code{run(p)}, \descriptor{} $p$ is not in the \code{active} status and if it is in the \code{won} status, its thunk has been run.
\end{lemma}

\begin{proof}
	The \code{decide(p)} on Line~\ref{line:decide} changes $p$'s status away from \code{active}. By  Lemma~\ref{lem:stableStatus}, once its status changes, it never changes again. Furthermore, \code{celebrateIfWon(p)} is called afterwards on Line~\ref{line:runCelebrateSelf}, which, if $p$'s status is \code{won}, runs $p$'s thunk.
\end{proof}

\begin{lemma}\label{lem:failed}
	If $p$ is in the \code{lost} state, its thunk is never run. Furthermore, a call to \code{run p.thunk} only happens after $p$ is in the \code{won} status.
\end{lemma}
\begin{proof}
	A thunk is run only in a call to \code{celebrateIfWon}. The \code{celebrateIfWon} function does not run a thunk if the \descriptor{}'s status is not \code{won}.
\end{proof}

\begin{lemma}
	If two calls \code{run p.thunk} and \code{run p'.thunk} are executed concurrently, neither \descriptor{} had its thunk run to completion earlier, and the lock sets of $p$ and $p'$ overlap, then $p = p'$. %\Naama{Adjust statement to allow concurrent thunk runs if an instance of one of them has already terminated.}
\end{lemma}

\begin{proof}
	Note that a \descriptor{}'s status can only change to \code{won} in the call to \code{decide(p)} on Line~\ref{line:decide} within a \code{run(p)} call, and that \code{run(p)} is only ever called after $p$'s priority is set to a non-negative value. 
	
	Assume by contradiction that $p \neq p'$, and let $\ell$ be a lock in the intersection of $p.lockSet$ and $p'.lockSet$. By Lemma~\ref{lem:failed}, both $p$ and $p'$ must have reached the \code{won} status. Without loss of generality assume that $p$ reaches the \code{won} status at time $w_p$, before $p'$. If $p$ is in $p'$'s set on Line~\ref{line:runGetSet} and $p'$ celebrates for $p$ after $w_p$, then $p$'s celebration, and thus the execution of its thunk, are completed before $p'$'s status is changed to \code{won} on Line~\ref{line:decide}.
	%
	We consider two cases.
	
	\textsc{Case 1.} $p'$ celebrates for $p$ before $w_p$. Then $p'$ must execute Line~\ref{line:compare} for $p$ before $p$'s reveal step, since otherwise $p'$ would have eliminated either itself or $p$, contradicting the assumption that they both eventually reach the \code{won} status. However, in this situation, since by assumption  $p$ reaches the \code{won} status first, $p$ must have $p'$ in its set when it executes Line~\ref{line:runGetSet}, and must have seen a non-negative priority for $p'$ and $p'$'s status as \code{active}. Therefore, $p$ would have eliminated one of the two, again contradicting our assumption that they both eventually execute their thunks.
	
	\textsc{Case 2.} $p'$ does not have $p$ in its set in Line~\ref{line:runGetSet}. Then by the correctness of the active set algorithm, $p$ must not have inserted  itself into the set yet. Similarly to the argument above, this means that $p$ must get $p'$ in its set when it executes Line~\ref{line:runGetSet}, and will observe $p'$ with a non-negative priority and an \code{active} status. Therefore, $p$ would eliminate one of the two \descriptor{s}, again contradicting the assumption that they both eventually execute their thunks.
\end{proof}

Therefore, the mutual exclusion property is maintained, and a thunk is run if and only if a \descriptor{} wins its tryLock. 
%\Naama{Should formally define the mutual exclusion property somewhere, and account for idempotence.}

\begin{theorem}
	Algortihm~\ref{alg:lock} satisfies the mutual exclusion with idempotence property (Definition~\ref{def:mutex}). Furthermore, if a tryLock attempt fails, then the corresponding thunk was never executed.
\end{theorem}

%\subsection{Fairness Proof}
%
%We say a \descriptor{} $p$ \emph{causes a \descriptor{} $p'$ to fail} if $p'$'s status is changed to \code{lost} in the \code{eliminate(p')} call on Line~\ref{line:eliminate1} or~\ref{line:eliminate2} after comparing $p'$'s priority with $p$'s priority. We say a \descriptor{} $p$ \emph{can cause $p'$ to fail} if $p$ and $p'$'s priorities are compared on Line~\ref{line:eliminate1} or~\ref{line:eliminate2} during the execution.
%
%\begin{lemma}\label{lem:differentLocks}
%	A \descriptor{} $p$ cannot cause a \descriptor{} $p'$ to fail if their lock sets do not intersect.
%\end{lemma}
%
%\begin{proof}
%	A \descriptor{} $p$ is only inserted into the sets corresponding to locks in its lock set (Line~\ref{line:insert}). Furthermore, in \code{run(p)}, only the sets of locks in $p$'s lock sets are compared against. Therefore, a \descriptor{} $p'$ will never be compared against and potentially eliminated by a \descriptor{} $p$ if their lock sets do not intersect.
%\end{proof}
%
%%\begin{lemma}\label{lem:endThreat}
%%	A \descriptor{} $p$ cannot cause a \descriptor{} $p'$ to fail if a \code{run(p)} call returned before $p'$'s reveal step.
%%\end{lemma}
%%
%%\begin{proof}
%%	First note that before $p'$'s reveal step, no \descriptor{} will eliminate $p'$, since its priority will be negative, and the comparison with it will be skipped on Line~\ref{line:compare}. Therefore, $p$ cannot cause $p'$ to fail before a \code{run(p)} returns. Furthermore, by Lemma~\ref{lem:doneStatus}, $p$'s status will not be \code{active}  after \code{run(p)} returns, and by Lemma~\ref{lem:stableStatus}, it will never be \code{active} again. Therefore, in any \code{run(p)} or \code{run(p')} call, the comparison of $p$ with any other \descriptor{} will be skipped on Line~\ref{line:checkActive}.
%%\end{proof}
%
%\begin{lemma}\label{lem:endThreat}
%	A \descriptor{} $p$ cannot cause a \descriptor{} $p'$ to fail if $p$'s status stopped being \code{active} before $p'$'s reveal step. 
%\end{lemma}
%
%\begin{proof}
%	First note that before $p'$'s reveal step, no \descriptor{} will eliminate $p'$, since its priority will be negative, and the comparison with it will be skipped on Line~\ref{line:compare}. Therefore, $p$ cannot cause $p'$ to fail before $p'$'s reveal step. By Lemma~\ref{lem:stableStatus}, $p$'s status will never be \code{active} again after it stops being \code{active}. Therefore, in any \code{run(p)} or \code{run(p')} call, the comparison of $p$ with any other \descriptor{} will be skipped on Line~\ref{line:checkActive} after $p$ becomes inactive. In particular, this comparison will always be skipped after $p'$'s reveal step.
%\end{proof}
%
%\begin{lemma}\label{lem:startThreat}
%	Let $p$ and $p'$ be  \descriptor{s} such that $p$'s tryLock starts after $p'$'s reveal step. Then neither \descriptor{} can cause the other to fail.
%	%A process $p$ cannot cause a process $p'$ to fail if $p$ starts its tryLock attempt after $p'$'s reveal step.
%\end{lemma}
%
%\begin{proof}
%	By Lemma~\ref{lem:differentLocks}, if $p$ and $p'$'s lock sets do not overlap, the lemma holds.
%	Otherwise, if $p'$ has already removed itself from the active set by the time $p$ started its \code{getSet} on Line~\ref{line:getHelpSet}, then $p'$ must have already won or lost by this time. In particular, $p$ wasn't in the active set during $p'$'s \code{run(p')}, and therefore could not have caused $p'$ to fail. Furthermore, by Lemma~\ref{lem:endThreat}, $p'$ cannot cause $p$ to fail.
%	
%	So, assume that $p'$ is still in the active set at the time $p$ started its \code{getSet} on Line~\ref{line:getHelpSet}. 
%	By the set regularity of the multi active set algorithm,
%	%By the linearizability of the active set algorithm, 
%	since $p'$ must have completed its insertion into the active set before $p$ started its \code{getSet} on Line~\ref{line:getHelpSet}, $p$ must have $p'$ in the set it gets. %Furthermore, since $p'$ already revealed its priority before $p$'s \code{getSet} linearized, $p$ must see a non-negative priority for $p'$. 
%	Therefore, $p$ calls \code{run(p')} before its own reveal step, so by Lemma~\ref{lem:doneStatus}, $p'$ wins or fails because of a different \descriptor{}. Furthermore, again by Lemma~\ref{lem:endThreat}, $p'$ cannot cause $p$ to fail, since a \code{run(p')} call completes before $p$'s reveal step, and therefore $p'$ is no longer active by that time.
%	%\Naama{Changed the code to run all processes in all sets, instead of just the highest priority ones.}
%	%There are two options.
%	%	
%	%	\textsc{Case 1.} $p'$ is added to the winner set directly, in which case $p$ will call \code{run(p')}. In this case, $p'$ will win or fail before any call to \code{run(p)}, and before $p$'s reveal step. Therefore, $p$ cannot cause $p'$ to fail. 
%	%	
%	%	\textsc{Case 2.} Some other process $q$ is added to $p$'s winners set on a lock that's in $p'$'s lock set. Then note that $q$ must be \code{active} at that time, and its priority must be higher than $p'$'s, by the way the winners are chosen. If $q$ and $p'$ are compared during the subsequent call to \code{run(q)} by $p$, then $p'$ will be eliminated because of $q$, and therefore $p$ will not cause its failure. If $q$ and $p'$ are not compared during that call, then either $q$ or $p'$ have moved to a status other than \code{active}. If it was $p'$, then the lemma holds; since $p$ has not revealed its priority yet, it could not have caused $p'$'s change of status. If $q$'s status was changed before $p$'s call to \code{run(q)} \Naama{to be continued. Might need to change code to actually execute run for everyone. I don't think it makes a big difference for running time.}
%\end{proof}
%
%We define the \emph{interval} of a \descriptor{} $p$ as the time between its calling process's call to tryLock and the time at which its tryLock call returns. Furthermore, a \descriptor{}'s \emph{threat interval} is the time between the beginning of its interval and the time at which its status stops being \code{active}.
%We define $p$'s \emph{threateners} as the set of \descriptor{s} that can cause $p$ to fail.
%% Given this definition and the lemmas above, we define $p$'s \emph{threateners} as the set of \descriptor{s} whose threat intervals overlap $p$'s reveal step.
%%
%%\begin{observation}\label{obs:threat}
%%	A \descriptor{} $p$ can cause a \descriptor{} $p'$ to fail only if $p$ is a threatener of $p'$.
%%\end{observation}
%%
%%\begin{proof}
%%	This is immediately implied by Lemmas~\ref{lem:endThreat} and~\ref{lem:startThreat}.
%%\end{proof}
%
%\begin{observation}\label{obs:threat}
%	The set of \descriptor{s} whose intervals overlap a \descriptor{} $p$'s reveal step includes all of $p$'s threateners.
%\end{observation}
%
%\begin{proof}
%	Every \descriptor{} $p$'s interval includes a complete call to \code{run(p)}. Thus, by Lemma~\ref{lem:doneStatus}, the status of any \descriptor{} is not \code{active} by the end of its interval. The lemma is therefore immediately implied from Lemmas~\ref{lem:endThreat} and~\ref{lem:startThreat}.
%\end{proof}
%
%\begin{observation}\label{obs:startPriority}
%	At the time at which a \descriptor{}'s interval starts, none of its threateners have reached their reveal step.
%\end{observation}
%
%\begin{proof}
%	This is immediate from Lemma~\ref{lem:startThreat}.
%	%	\Naama{Maybe change definition of threatener to be anyone whose priority gets compared to that of $p$, and change Obs~\ref{obs:threat} to say that the set whose intervals overlap with $p$'s reveal step includes all threateners. Shouldn't have to change lemma statements/proofs much, and might be easier to talk about.}
%\end{proof}
%
%\begin{observation}\label{obs:constantSteps}
%	Each \descriptor{} interval takes the same number of steps by the initiating process between its start and its reveal step, and between its reveal step and the end of its interval, regardless of the schedule or randomness.
%\end{observation}
%
%\begin{proof}
%	This property is enforced by the delays injected in Lines~\ref{line:delay1} and~\ref{line:delay2}.
%\end{proof}
%
%%\Naama{Sketch of the rest of the proof}
%
%We say  that a \descriptor{} $p$ is a \emph{potential threatener} of another \descriptor{} $p'$ if (1) $p$'s interval overlaps with $p'$'s reveal step, and (2) $p'$ did not execute a \code{run(p)}. Note that by Observation~\ref{obs:threat} and Lemma~\ref{lem:endThreat}, the set of potential threateners of a \descriptor{} is a superset of its actual threateners. 
%%We say  that a \descriptor{} $p$ \emph{contends} with another \descriptor{} $p'$ if $p$'s interval overlaps with $p'$'s reveal step. Note that the contend relationship is not symmetrical.  Furthermore, note  that the set of contenders of a \descriptor{} is a superset of its threateners, by Observation~\ref{obs:threat}.
%
%%\begin{lemma}
%%	Adversarial choices that affect whether $p$ will threaten $p'$ must happen before the adversary knows anything about either \descriptor{}'s priority.
%%\end{lemma}
%
%\begin{lemma}\label{lem:pairwiseIndep2}
%	The player adversary does not have any information on the priorities of $p$ or $p'$ at the time at which it decides to make $p'$ threaten $p$.
%	%The event that $p$ is a potential threatener of $p'$ in an execution $E$ is independent of both $p$ and $p'$'s priorities. 
%	%\Naama{Problem: if $p$ is really slow and is not taking any steps, $p'$ can contend with it even if it joined after $p$'s reveal step. However, it won't be threatened by $p$. The problem is that we can't use threatening as the relationship in the claim here either, because depending on $p$'s priority, it may stop being a threatener very early on. Could solve this by removing someone from its locks as part of helping them. Then define the interval as the time you are in the active set of any lock. Do we need that?}
%\end{lemma}
%
%\begin{proof}
%	By Observation~\ref{obs:constantSteps}, once a \descriptor{} starts, its reveal step and last step of its interval are determined. Since these two steps are what determines whether a \descriptor{} will be a potential threatener of  another \descriptor{}, the start times of the two \descriptor{s} determine whether this event occurs. 
%	Furthermore, by Lemma~\ref{lem:startThreat} and the definition of potential threateners, if $p$ is a potential threatener of $p'$ in an execution $E$, then both $p$ and $p'$ must have started their tryLock interval before either of their reveal steps. Therefore, the player adversary did not have any information on their priorities at the time at which it decided to start their intervals. 
%	%Therefore the event that $p$ is a potential threatener of $p'$ is independent of both of their priorities.
%\end{proof}
%
%\begin{theorem}
%	Let $k_\ell$ be the bound on the maximum point contention possible on lock $\ell$, and let $C_p = \sum_{\ell \in p.lockList} k_\ell$ be the sum of the bounds on the point contention across all locks in a \descriptor{} $p$'s lock list. Then there exists an algorithm $A$ for wait-free fine-grained locks against an oblivious scheduler and an adaptive player such that the probability that $p$ succeeds in its tryLock in $A$ is at least $\frac{1}{C_p}$.
%	%The probability that \descriptor{} $p$ succeeds in its tryLock is at least $\frac{1}{CL}$. \Naama{Bound can have lower case $\ell$, i.e., the actual number of locks taken, instead of the maximum.}
%\end{theorem}
%
%
%\begin{proof}
%	On each lock $\ell$ in $p$'s lock list, the adversary can make at most $k_\ell$ \descriptor{s} be potential threateners of $p$. Assume that all priorities of the \descriptor{s} are picked uniformly at random, but the priority of a given \descriptor{} $p'$ is hidden until after the adversary chooses whether or not $p'$ will be a potential threatener of $p$. This is equivalent to our setting since the priorities are always picked uniformly at random, and, by Lemma~\ref{lem:pairwiseIndep2}, the adversary has no information on a \descriptor{} $p'$'s priority until after it decides whether it will potentially threaten $p$. Once the adversary discovers the priority of a \descriptor{}, it can decide whether the next \descriptor{} will be a potential threatener of $p$ and then reveal the corresponding priority. In the worst case, the adversary can reveal up to $C_p$ of those predetermined priorities. Since the set of potential threateners of $p$ include all actual threateners of $p$, this makes $p$ threatened by $C_p$ uniformly chosen random values in the worst case, giving it a $\frac{1}{C_p}$ probability of having the maximum priority of all of them.
%\end{proof}


==> multi-wwm.tex <==
\section{Nesting the Lock Algorithm}

Lock algorithms often need to be nested within themselves in complex programs. For example, in transactional memories, a transaction must often hold a lock on several locations at once to ensure that it can complete its execution atomically. 
Thus, in this section we modify Algorithm~\ref{alg:single-lock} to allow it to be nested within itself. There are two main challenges here: firstly, Algorithm~\ref{alg:single-lock} only works for idempotent thunks, but is not idempotent itself. Secondly, nesting locks may threaten the running time and fairness guarantees that Algorithm~\ref{alg:single-lock} provides.
% requires the code within the lock (i.e. the thunks described by the announced descriptors) to be idempotent. However, the algorithm itself is not idempotent.
%We therefore present an idempotent version Algorithm~\ref{alg:lock} in this section.
%
In particular, helping another descriptor complete its thunk may involve helping it grab another lock, which in turn may require helping another process complete its own thunk. In this way, a chain of helping can appear, blowing up the cost of attempting to grab a single lock from constant to linear in the size of the data structure. \Naama{Instead of constant, we can call it `proportional to the length of a thunk'.} Furthermore, if a descriptor only accesses a certain lock if it already successfully grabbed a previous one, it may skew the priorities that a descriptor competes with, thus breaking the fairness guarantees.

In this section, we address these issues.  \Naama{Merge between the texts above and below.}
%We first show how to maintain good step complexity and fairness bounds when attempting to grab the lock, and later discuss how to make the lock idempotent.



%\subsection{Making an Idempotent Write-with-Max}
%
%\begin{figure}\label{alg:wwm}
%	\begin{lstlisting}
%	Descriptor[k] announce;
%	
%	void advancePredecessor(int slot){
%	for (int i=0; i<2; i++){
%	Descriptor pred = announce[slot+1];
%	Descriptor cur = announce[slot];
%	if (pred @$\neq$@ null){
%	CAS(announce[slot], cur, pred);	}	}
%	}
%	
%	void writeWithMax(Descriptor myDesc, int priority){
%	if (announce[priority+1] == null){
%	CAS(announce[priority], null, myDesc);	}
%	mySlot = priority;
%	while(mySlot @$\geq$@ 1){
%	advancePredecessor(mySlot);
%	mySlot -= 1;	}
%	}
%	
%	void clear(Descriptor myDesc, int priority){
%	for (int i=priority; i>0; i--){
%	CAS(announce[i], myDesc, null);	}
%	}
%	\end{lstlisting}
%	\caption{Idempotent Write-with-Max}
%\end{figure}



We now consider a scenario in which a process must acquire several locks before executing some inner thunk. 
%We assume that each process's descriptor now contains, aside from the thunk, a list of locks to be acquired. To execute a given descriptor,  a process must first ensure that the locks in the list have all been acquired, in order. 
Note that using Algorithm~\ref{alg:single-lock}, a process $p_1$ attempting to grab a lock may end up helping to execute the descriptor of another process, $p_2$ (whose priority was already in the \texttt{live} slot). Thus, $p_1$ will attempt to acquire the next lock that $p_2$'s descriptor needs. However, when acquiring $p_2$'s next lock, $p_1$ may have to help another process, $p_3$. This can continue in an arbitrarily long chain of locks that $p_1$ would need to help acquire, even if each individual descriptor only requires a constant number of locks. Furthermore, if  losing on a lock attempt causes $p_1$ to give up on trying to acquire its other locks, %if $p_1$  does compete on other locks, 
$p_1$'s its conditional priority is no longer distributed uniformly in the same range as originally.

We present a nesting algorithm that avoids these issues. For this algorithm, we also require the use of a different wwm algorithm, which would allow use to concurrently announce a descriptor's priority on many locks at once. For this purpose, we begin by presenting an implementation of wwm that allows us to do so.



\subsection{Multi-location WWM}

We modify the universal construction of Afek et al.~\cite{afek1995wait} to allow us to execute a wwm concurrently on \emph{several locations at once}. In Afek et al.'s algorithm, processes announce their descriptor by scanning an announcement array of length $n$, and \emph{capturing} the first available slot by placing their descriptor in it. They then `climb' in the array, trying to place their descriptor in each slot from the one they \\capture{}{}d to the first in the array, recursively helping any descriptor they encounter along the way. 

To allow executing a wwm on several locations at once, we modify the algorithm to have a \emph{ready} flag in each descriptor. We announce the descriptor, with the ready flag set to false, on all the wwm objects we need, and then change the ready flag to true.  Processes helping the announcements in each wwm object skip announcements whose flag is false. The pseudocode for this algorithm is presented in Algorithm~\ref{alg:wwm}, with the modifications over Afek et al.'s algorithm highlighted in green.

\begin{figure}
	\begin{lstlisting}
struct Descriptor{
	bool ready;
	bool done;
	T op_descriptor;
}
<Descriptor, bool>[] Ann;

int findSlot(Descriptor desc){
	for (int i=0; i< P; i++){
		if (CAS(Ann[i], null, desc)){
			return i;	}	}
}

int, bool findParent(int index){
	return ((index/2), (index mod 2));
}

void climb(Descriptor desc, int parent, bool direction){
	if (parent == 0){
		Execute(desc.op_descriptor);
		desc.done = true;	
		return;	}
	bool finished = false;
	next, dir = findParent(parent);
	while (true) {
		cur, cur_dir = Read(Ann[parent]);
		if (cur == null){
			CAS(Ann[parent], null, (desc,dir));	}
		if (cur == desc){
			climb(desc, next, dir);
			return;	}
		if (not cur.ready){
			if (CAS((cur, cur_dir)))
			climb(desc, next, dir);
			finished = true;
			return;	}
		else if (cur.done) {
			release(parent);	}
		if (finished){ return; } //important to prevent blowup to @$P^2$@ time if there are many not-ready
		else if (cur == read(Ann[parent])){
			climb(cur, next, dir);	}
	}
}

void realse(index){
	for (int i=0; i<2; i++){
		cur, cur_dir = read(Ann[index]);
		if ((cur == null) || (not cur.done)){	return; }
		bool ok = false;
		Descriptor prev;
		int j = index;
		while (not ok){
			prev = read(Ann[j+1]);
			if ((prev != null) && (not prev.ready)) {
				j++;}
			else { ok = true;	}		}
		CAS(Ann[index], cur, prev);
	}
}

void operation(T op_descriptor, bool* ready){
	Descriptor desc = {*ready, false, op_descriptor};
	int index = findSlot(desc);
	while(not *ready){};
	desc.ready = true;
	climb(desc, index-1);
	for (int i=index; i>= 0; i--){
		release(i);
	}
	
@\Naama{Currently the code is half for tree structure, half for array. The array yields $k^2$ running time, where $k$ is the point contention. I haven't quite figured out how to do the tree structure one, since it requires successfully skipping over descriptors that aren't ready.}
}
	\end{lstlisting}
\end{figure}


\begin{lemma}
	Once you return from a \texttt{climb(desc, 1)} call, you never recurse again.
\end{lemma}

\Naama{TODO: show pseudocode for multi-wwm, prove it works.}

We note that our algorithm does not produce a linearizable multi-location wwm. Instead, it guarantees the following \emph{regularity} property.
\begin{property}
	Consider a multi-location wwm operation $op$ with lock set $\mathcal{L}$ that set its ready flag to true at time $t$. Then on each lock $\ell \in \mathcal{L}$, any wwm operation $op'$ that starts after time $t$ will linearize after $op$. 
\end{property}

Intuitively, wwm operations must linearize in the order of timing of their \emph{\capture} intervals; a wwm operation $op$ whose \capture{} interval ends before the \capture{} interval of some operation $op'$ begins will linearize before $op'$ on every lock that $op$ and $op'$ have in common.

Furthermore, another important property of the wwm algorithm is that the linearization of each operation on each object is independent of that operation's values other than its ready flag. In particular, the linearization point of an operation $op$ on a wwm object does not depend on $op$'s descriptor's priority.

\begin{property}
	The linearization point of an operation $op$ does not depend on the operation itself. \Naama{Formalize this.}
\end{property}

\begin{property}
	An operation $op$ cannot be linearized on any object until the ready flag in its descriptor is set to true.
\end{property}

==> multiactiveproofs.tex <==
\section{Multi Active Set Correctness and Step Complexity Proofs}\label{sec:multiactiveproofs}

\begin{theorem}[Theorem \ref{thm:multisetCorrectness}.]
	The Multi Active Set algorithm presented in Algorithm~\ref{alg:multiactive} satisfies set regularity, assuming it uses a linearizable Active Set implementation.
\end{theorem}

\begin{proof}
	Let the linearization point of a \minsert{} operation be at its setFlag. Let the linearization point of a \mremove{} be at its clearFlag.
	We need to show that (1) any getSet of set $S$ that starts before the linearization of an \minsert$(I, C)$ where $S \in C$ will not include $I$ in its return set, (2) any getSet of set $S$ that starts after the linearization of an \minsert$(I, C)$ where $S \in C$ and returns before the linearization point of the corresponding \mremove{} returns a set that includes $I$, and (3) any getSet of $S$ that begins after the linearization of the \mremove{} will not include $I$ in its set.
	To see this, note that an item whose flag is false is not returned in a getSet. Thus, (1) and (3) hold since each item's flag is cleared at the beginning of a \minsert{}, before the \minsert's linearization, and is also cleared at the linearization of the corresponding \mremove{}, and is not set to true after that point. Thus, a getSet that returns before the linearization of a \minsert{} or begins after the linearization of a \mremove{} cannot return the relevant item.
	
	To see (2), note that an \minsert{} calls setFlag after calling insert on each of the sets in the collection $C$. Thus, since the underlying active sets are linearizable, the insert into each set has linearized by this point. Furthermore, the only remove operations called on the underlying active sets are through the \mremove{} operation, after it calls clearFlag. Thus, between the linearization of a \minsert$(I, C)$ and the linearization of the corresponding \mremove{}, S.getSet on any $S\in C$ will return $I$, by the linearizability of the underlying active set. Furthermore, since the flag of $I$ is set at the linearization point of the \minsert{} and not cleared until the linearization point of the \mremove, a getSet$(S)$ will not remove $I$ from the set returned by the multi active set.
\end{proof}

\begin{theorem}[Theorem \ref{thm:multisetTime}.]
	In Algorithm~\ref{alg:multiactive}, each operation takes $O(\kappa)$ steps per active set it accesses.
\end{theorem}

\begin{proof}
	Using Algorithm~\ref{alg:activeSet} as the underlying active set object, each insert and remove operation takes $O(\kappa)$ steps. Therefore, the theorem holds for \minsert{s} and \mremove{s}, each of which simply calls insert or remove (respectively) on each active set it accesses. 
	The getSet method accesses only one active set, and iterates over each returned element once. Since the active set's getSet method takes constant time and returns a set of size at most $\kappa$,  the multi active  set's getSet takes $O(\kappa)$ steps.
\end{proof}

==> nestedProofs.tex <==
\section{Nested Lock Proofs}\label{sec:nestedProofs}

\subsection{Safety}


\begin{lemma}\label{lem:noStatusChange}
	Once a descriptor's status is \texttt{safe} or \texttt{aborted}, it does not change.
	%, its status cannot change to \texttt{aborted}. Furthermore, once a descriptor's status is \texttt{aborted}, its status cannot change to \texttt{safe}. 
\end{lemma}

\begin{proof}
	A descriptor $d$'s status gets changed in only two places in the code: (1) in the \texttt{tryAbort} function, and (2) in the \texttt{tryProtect} function.
	%, and (3) on Line~\ref{line:writeDone}. 
	Both (1) and (2) change $d$'s status through a CAS whose old value is \texttt{active}, with a new value that is not \texttt{active}. %In (3), the value gets changed to \texttt{done}. 
	Therefore, once $d$'s status changes away from \texttt{active}, it never goes back to that value. 
	The only way for $d$'s status to change to \texttt{aborted} is through (1); by the above, if its status was already changed to \texttt{safe}, the CAS in \texttt{tryAbort} will always fail, and therefore the status cannot change to \texttt{aborted}. 
	Similarly, if $d$'s status is already \texttt{aborted}, it can never change to \texttt{safe}, since the CAS in \texttt{tryProtect} will always fail.
	%to \texttt{safe} only through the function \texttt{tryProtect}. In \texttt{tryProtect}, a CAS is executed with old value \texttt{active}. Therefore, if a 
\end{proof}

\begin{lemma}
	A descriptor $d$'s thunk cannot start being executed at time $t$ unless $d$'s status was \texttt{safe} at some time $t < t'$.
\end{lemma}

\begin{proof}
	A descriptor $d$'s thunk is only executed in Line~\ref{line:runThunk}. This line only gets executed if the check on Line~\ref{line:safeCheck} passes, that is, if \texttt{d.protected()} returns true. This only happens if $d$'s status is \texttt{safe}.
\end{proof}

\begin{lemma}\label{lem:liveRemovalStatus}
	A descriptor gets removed from the \texttt{live} slot only under two conditions: either its status is \texttt{aborted}, or its status is 
	%\texttt{done}, 
	\texttt{safe}, and its thunk has already been executed.
\end{lemma}

\begin{proof}
	Let $d$ be a descriptor that is written in the \texttt{live} slot of a lock $\ell$ at time $t$. 
	A CAS that changes the \texttt{live} slot happens in three places in the code. Two of them are immediately after running \texttt{d.helpDescriptor}. Since \texttt{d.tryProtect} is called in \texttt{d.helpDescriptor}, $d$ must be either safe or aborted when that function returns. 
	The other place that a CAS on \texttt{live} is called is in Line~\ref{line:CASliveIfAborted}, which ensures that $d$ is aborted before the CAS is executed.
	%	
	%	The \texttt{live} slot is changed on Line~\ref{line:liveCAS} of $\ell$'s \texttt{compete} function, with a CAS whose old value is returned from a \texttt{helpLive} call, which is only executed if all of the following conditions hold: (1) the descriptor in the \texttt{docket} is not safe, (2) the descriptor \texttt{desc} is not safe, (3) \texttt{isInitiator} is true. 
	%	If the CAS \textit{is} executed, for it to remove $d$ from \texttt{live}, $d$ must have been returned as the second value from \texttt{helpLive}. Therefore, \texttt{helpLive} ran with $d$ as its \texttt{liveVal}.
	%	%Since the \texttt{helpLive} function returns the descriptor it helped, $d$ must have been helped before it gets removed from \texttt{live}. 
	%	
	%	Note that in \texttt{helpLive}, \texttt{d.helpDescriptor} is called if \texttt{d} is not aborted, and additionally,  the conditions listed above are satisfied. 
	%	If \texttt{d} did get aborted, then the lemma is satisfied.
	%	Otherwise, if the CAS on Line~\ref{line:liveCAS} was executed, then \texttt{d.helpDescriptor} was also executed. Note that during \texttt{d.helpDescriptor}, \texttt{d.tryProtect} is called on Line~\ref{line:tryProtect}. If this call successfully made $d$ safe, then Line~\ref{line:runThunk} will be executed, and $d$'s thunk will be run before returning from \texttt{helpDescriptor}, and in particular, before returning from \texttt{helpLive}. Therefore, when the CAS on Line~\ref{line:liveCAS} was executed, $d$ is safe and its thunk was executed.
	%	If the \texttt{tryProtect} call on Line~\ref{line:tryProtect} does not change $d$'s status to safe, then by Lemma~\ref{lem:noStatusChange}, $d$ was aborted. This also satisfies the conditions of the lemma.
\end{proof}
%
%\begin{lemma}\label{lem:abortBeforeHelp}
%	If \texttt{d.helpDescriptor} is called for some descriptor $d$ at time $t$ during the execution of a \texttt{compete(d')} call for some descriptor $d'$, then either (1) $d'$ is aborted by $t$, or (2) $d$ is safe by $t$. 
%\end{lemma}
%
%\begin{proof}
%	%We first note that if $d = d'$, then the \texttt{helpLive} function returns without calling \texttt{helpDescriptor} (Line~\ref{line:returnIfSelf}), so this case is irrelevant for the lemma. 
%	
%	We consider two cases; either $d'$ is the descriptor returned when the \texttt{docket} is read on Line~\ref{line:readDocket}, or it isn't. 
%	
%	%Case 1. $d'$ is the descriptor returned when the \texttt{docket} is read on Line~\ref{line:readDocket}. 
%	Note that \texttt{d.helpDescriptor} is called in two places; Line~\ref{line:helpDescSafe} and Line~\ref{line:helpDescInit}. Note that Line~\ref{line:helpDescSafe} is only called if $d$ is safe, so this satisfies the lemma. If \texttt{d.helpDescriptor} is called on Line~\ref{line:helpDescInit}, then note that $d'.tryAbort$ has been called on $d'$, either on Line~\ref{line:abortDocket} or Line~\ref{line:abortNotInDocket}. If this call aborted $d'$, then we are done.
%	\Naama{Is it ok to let $d'$ be potentially safe, and not just aborted? Otherwise, need to think of argument and possibly modify code.}
%%	
%%	Note that \texttt{d.helpDescriptor} is called on Line~\ref{line:callHelpDesc}, only if $d$ is not aborted when its status is checked on Line~\ref{line:checkAborted}. We consider two subcases, depending on whether or not $d$'s priority is higher than $d'$'s priority. If it is, then \texttt{tryAbort} gets called on $d'$ on Line~\ref{line:abortDocket}. Thus, $d'$ must either be safe or aborted after this time. Furthermore, if $d'$ is \texttt{safe}, then the check on Line~\ref{line:checkAborted} fails, and it does not help $d$.
%%	If $d'$'s priority is higher than $d$'s priority, then \texttt{tryAbort} is called on $d$ on Line~\ref{line:tryAbortLock}. Thus, $d$ must be either safe or aborted after this time. If it is aborted, then Line~\ref{line:callHelpDesc} would not have been called, contradicting the lemma assumption.
%%	
%%	Case 2. $d'$ is not the descriptor returned when the \texttt{docket} is read on Line~\ref{line:readDocket}.
%%	Then \texttt{tryAbort} is called on $d'$ on Line~\ref{line:abortNotInDocket}. If it aborts $d'$, then the lemma holds. Otherwise, by Lemma~\ref{lem:noStatusChange}, it must be safe, so the \texttt{helpLive} fails its check on Line~\ref{line:checkAborted}, and does not call \texttt{helpDescriptor}.
%\end{proof}

\begin{lemma}\label{lem:competeStatus}
	A descriptor $d$ 
	is either in the \texttt{live} slot of a lock $\ell$, or it 
	is no longer in the \texttt{active} status when a \texttt{compete(d)} call on $\ell$ returns.
\end{lemma}

\begin{proof}
	By Lemma~\ref{lem:CasInLoop}, a successful CAS of the \texttt{live} slot with a new value that was read from the docket after $d$'s \wwm{} must have occurred before the \texttt{compete(d)} returned.
	
	Note that this CAS must have used as its new value the \texttt{dock} descriptor returned from a \texttt{helpLive} call. If $d$ was the new value in this CAS, then $d$ was put in the \texttt{live} slot at this point. By Lemma~\ref{lem:liveRemovalStatus}, if $d$ was removed from \texttt{live} before the end of the \texttt{compete}, then it is no longer \texttt{active}. Otherwise, it is still in \texttt{live}, and the lemma is also satisfied.
	
	So, we consider the case in which $d$ was not the new value in this CAS. Then in the \texttt{helpLive(d)} that return the new value, $d$ was not the \texttt{dockVal}, so \texttt{d.tryAbort} was executed on Line~\ref{line:abortNotInDocket}. Therefore, it can no longer be \texttt{active}.
	%
	%	If the \texttt{compete(d)} instance called \texttt{helpDescriptor}, then it either called \texttt{d.tryAbort}
	%	By Lemma~\ref{lem:abortBeforeHelp}, if the \texttt{compete(d)} instance called \texttt{helpDescriptor}, then $d$ was not \texttt{active} at the time of that call, and by Lemma~\ref{lem:noStatusChange}, it remains that way when the \texttt{compete(d)} returns. We therefore consider the cases in which a \texttt{compete(d)} does not call \texttt{helpDescriptor}. 
	%	
	%	This can happen for two reasons (1) $d == liveVal$ in Line~\ref{line:returnIfSelf}, and (2) the \texttt{liveVal} was aborted when checked on Line~\ref{line:checkAborted}. In case (1), by Lemma~\ref{lem:liveRemovalStatus}, $d$ must either still be on \texttt{live} when \texttt{compete(d)} returns, or it must already be either \texttt{safe} or \texttt{aborted}. In case (2), since $d$ was not aborted on Line~\ref{line:abortNotInDocket}, $d$ must have been on the docket. By Lemma~\ref{lem:CasInLoop}, a successful CAS of the \texttt{live} slot with new value $d$ must have occurred before the \texttt{compete(d)} returned.
\end{proof}

\begin{lemma}\label{lem:safeHoldsLocks}
	A descriptor $d$'s status cannot change to \texttt{safe} unless it is in the \texttt{live} slot of each lock in its \texttt{lockList}.
\end{lemma}

\begin{proof}
	Note that the only place in the code in which a descriptor $d$'s status can be changed to \texttt{safe} is on Line~\ref{line:tryProtect}. This line is only executed after $d$ has competed on each of its locks. Consider the first process $p$ that executes this line for $d$. For each lock $\ell$ in $d$'s \texttt{lockList}, if $d$ was not in $\ell$'s \texttt{live} slot immediately after $p$ competed on it,  the by Lemma~\ref{lem:competeStatus}, it must not have been \texttt{active} by that time. Since $p$ is the first to execute Line~\ref{line:tryProtect} for $d$, and this is before it does so, $d$ could not have become \texttt{safe}, so it must have been \texttt{aborted} in this case. %then $p$ would have changed $d$'s status to \texttt{aborted} on Line~\ref{line:abortself}. 
	%Since $p$ is the first process to execute Line~\ref{line:tryProtect} for $d$, its \texttt{tryAbort} before Line~\ref{line:tryProtect} must see its status as \texttt{active} or \texttt{aborted}, and therefore, after $p$ executes \texttt{tryAbort}, $d$'s status will be \texttt{aborted}. 
	By Lemma~\ref{lem:noStatusChange}, $d$'s status will never become \texttt{safe} if this happens.
	
	Therefore, if $d$'s status ever becomes \texttt{safe}, for each lock $\ell$ in its \texttt{lockList}, $d$ must have been in $\ell$'s live slot at some point before $d$ become \texttt{safe}. By Lemma~\ref{lem:liveRemovalStatus}, $d$ can only be removed from a lock's \texttt{live} slot if its status is \texttt{safe} or \texttt{aborted}. If it is removed when its status is \texttt{safe}, we are done. Otherwise, if its status became \texttt{aborted}, by Lemma~\ref{lem:noStatusChange}, it can never become \texttt{safe}.
\end{proof}

\begin{lemma}\label{lem:holdAllLocks}
	A descriptor $d$'s thunk cannot get executed unless $d$ holds all locks in its \texttt{lockList}.
\end{lemma}

\begin{proof}
	$d$'s thunk only ever gets executed on Line~\ref{line:runThunk}, which is only executed if the check on Line~\ref{line:safeCheck} shows that $d$'s status is \texttt{safe}. By Lemma~\ref{lem:safeHoldsLocks}, if $d$'s status is \texttt{safe}, then it held all of its locks at some point. Furthermore, by Lemma~\ref{lem:liveRemovalStatus}, after this point, it cannot get removed from any lock until after its thunk is executed. Therefore, $d$ must still hold the locks while its thunk gets executed for the first time.
	Since $d$'s thunk must be idempotent, all thunk executions after the first have no effect.
\end{proof}

\begin{lemma}\label{lem:notActive}
	When a call to \texttt{tryLocks} returns, the status of the descriptor $d$ that was created for this call cannot be \texttt{active}.
\end{lemma}

\begin{proof}
	The \texttt{tryLocks} function calls \texttt{helpDescriptor}, which calls \texttt{compete(d)}. By Lemma~\ref{lem:competeStatus}, after each \texttt{compete}, $d$'s status is either no longer \texttt{active}, or $d$ is in the \texttt{live} slot of the corresponding lock. In the first case, we are done. In the second, note that \texttt{tryProtect} (Line~\ref{line:tryProtect}) during the execution of the \texttt{helpDescriptor} function, after all the \texttt{compete} calls. If this call changes $d$'s state, we are also done. If not, its CAS failed. However, the CAS in \texttt{tryProtect} has old value \texttt{active} and operates on the \texttt{status} field of $d$. If it fails, then $d$'s status must not be \texttt{active} at that time. Again by Lemma~\ref{lem:noStatusChange}, $d$'s status cannot have returned to \texttt{active}.
	%	
	%	which must call either \texttt{tryAbort} (Line~\ref{line:abortself}) or \texttt{tryProtect} (Line~\ref{line:tryProtect}) during its execution. If one of these calls changes the status of $d$, then by Lemma~\ref{lem:noStatusChange}, we are done. If these calls do not change the status, then their CASes must have failed. However, the CAS in both \texttt{tryAbort} and \texttt{tryProtect} have old value \texttt{active} and operate on the \texttt{status} field of $d$. If they fail, then $d$'s status must not be \texttt{active} at that time. Again by Lemma~\ref{lem:noStatusChange}, $d$'s status cannot have returned to \texttt{active}.
\end{proof}

\begin{lemma}\label{lem:correctReturnVal}
	A thunk gets executed if and only if its \texttt{tryLocks} call returns true, in which case it is executed before the call returns.
\end{lemma}

\begin{proof}
	By Lemma~\ref{lem:notActive}, the descriptor $d$ that was created during the execution of \texttt{tryLocks} cannot have status \texttt{active} when the call terminates. By Lemma~\ref{lem:noStatusChange}, the status can only change once. By Line~\ref{line:safeCheck}, a thunk gets executed only if its status is \texttt{safe}. In this case, the thunk is executed before the end of the \texttt{helpDescriptor} function, which returns before \texttt{tryLocks} returns. Furthermore, \texttt{tryLocks} returns true in this case, and in no other cases. 
\end{proof}

Lemmas~\ref{lem:holdAllLocks} and~\ref{lem:correctReturnVal} together immediately imply the following theorem about the correctness of the nested lock algorithm.

\begin{theorem}
	In Algorithm~\ref{alg:nestedlock-lock}, if a thunk gets executed, then this happens while its descriptor holds all of the locks provided to the \texttt{tryLocks} function, and before the function returns. Furthermore, the function returns true if and only if the thunk got executed.
\end{theorem}


\subsection{Fairness}


%on some lock in $L \cap L'$ overlaps $d'$'s danger interval. %Note that the threat interval of a descriptor $d$ ends at a different time on each of its locks.
%For the definition of \emph{blame} (Definition~\ref{def:blame}), we keep the same notion, but consider it on a per-lock basis rather than the entire operation; more precisely, we say that a descriptor $d$ \emph{blames} descriptor $d'$ on lock $\ell$  if $d'$ is returned by $d$'s \firstcritread{} on $\ell$.
We now show that the nested lock algorithm preserves some of the properties of the single-lock algorithm that helped reason about fairness. 

%
%\begin{lemma}\label{lem:nested-blame}
%	If a descriptor $d'$ is returned in the \firstcritread{} of a descriptor $d$ on lock $\ell$, 
%	%If descriptor $d$ blames descriptor $d'$ on lock $\ell$ 
%	then $d'$ threatens $d$ on $\ell$ and $d'$'s priority is higher than $d$'s. 
%	%\Naama{change phrasing to avoid `blame' and only talk about being in docket during the \firstcritread. Then use this in the lemma above (so move it up). Possibly redefine blame to mean the person who caused you to abort (still would leave this lemma as not directly blame)}
%\end{lemma}
%
%\begin{proof}
%	This claim's proof is very similar to the analogous claim for the single-lock version (Claim~\ref{clm:blame}), and derives directly from the definitions of blame and threat. 
%	Let $t$ be the time at which $d$'s \firstcritread{} is executed on $\ell$.
%	$d'$'s descriptor must be written in the \texttt{docket} of $\ell$ at $t$. Note that if $d'$ doesn't threaten $d$ on $\ell$, then either (1) its threat interval ended before $d$'s danger interval began, or (2) its threat interval started after $d$'s \dangerInt{} ended. 
%	In case (1), then either $d'$ is aborted before $d$'s danger interval began, or its \assocClear{} already  happened. By Claim~\ref{clm:cleared}, if $d'$'s \assocClear{} already  happened, then $d'$ cannot be in the docket afterwards. We note that the Claim~\ref{clm:cleared} applies to the nested lock algorithm, since it depends on parts of the algorithm that remain the same between the single and the nested versions. 
%	Note that by Claim~\ref{clm:univ} $d$'s danger interval starts before its wwm linearizes on any lock. If $d'$ aborted, then by the definition of the multi-wwm, $d$ cannot lose its wwm to $d'$. 
%	
%	In case (2), recall that $d$'s \dangerInt{} ends after its \firstcritread{} on every lock, since its \dangerInt{} ends at its first \texttt{tryProtect}, which is only called from a \texttt{helpDescriptor} instance for $d$, after ensuring $d$'s wwm linearized and competing on each lock.
%	% by Lemma~\ref{lem:safeHoldsLocks}, $d$ cannot become safe before it is on the \emph{live} slot on all of its locks \Naama{Need to refine argument to include the option that the tryProtect fails}. 
%	Therefore, in particular, $d$'s \dangerInt{} ends after $t$. Thus, $d'$'s threat interval must have started after $t$. However, recall that the threat interval starts when $d'$'s ready flag is set to true. By Claim~\ref{clm:univ}, $d'$ cannot already be in the \texttt{docket} of any lock before its ready flag is set. Therefore, it cannot be returned by a read of the \texttt{docket} of $\ell$ at time $t$. 
%	
%	Furthermore, note that $t$ must be after both descriptors had their wwm linearized on $\ell$, but before their \assocClear. Additionally, \Naama{need to claim $d$ wasn't already aborted. Can we make $d$'s danger interval end when it gets aborted?}
%	By the correctness of wwm, if $d'$ is written in \texttt{docket} at that time, then $d'$'s priority is higher.
%\end{proof}
\begin{lemma}\label{lem:nested-early-end}
	If a descriptor $d$ threatens a descriptor $d'$ and $d'$'s danger interval started after $d$'s danger interval, then $d$'s danger interval ends before $d'$'s \activeInt{} ends.
	%	If a descriptor $d$ threatens a descriptor $d'$ and either (1) 
	%	$d'$'s \activeInt{} started after $d$'s threat interval started, or (2) $d$ was returned in $d'$'s \firstcritread, 
	%	then, on all of $d'$'s locks, $d$'s threat interval ends at the same time as or earlier than the \activeInt{} of $d'$ on that lock.
\end{lemma}

\begin{proof}
	Consider a lock $\ell$ which was on both $d$ and $d'$'s \texttt{lockList}. By Claim~\ref{clm:univ}, since $d'$'s ready flag was set to true after $d$'s ready flag and $d'$ executed \texttt{helpAll} after that point, $d$'s \wwm{} linearized on $\ell$ before $d'$'s read of \texttt{docket} on $\ell$. We consider three cases, based on which descriptor is returned in lines~\ref{line:readDocket} and~\ref{line:readLive} of $d'$'s \texttt{compete(d', true)} call (which must have been called by $d'$'s initiator).
	
	Case 1. $d$ is returned in the read of \texttt{live} on Line~\ref{line:readLive} in one of the \texttt{helpLive} calls in  \texttt{compete(d', true)} on $\ell$. Then, since \texttt{isInitiator == true}, some CAS on \texttt{live} replaces $d$ with another descriptor by the end of this \texttt{helpLive}. By Lemma~\ref{lem:liveRemovalStatus}, $d$ must be \texttt{aborted} or \texttt{safe} when that happens, so its danger interval is over.
	
	Case 2. $d$ is returned in the read of \texttt{docket} on Line~\ref{line:readDocket} in one of the \texttt{helpLive} calls in  \texttt{compete(d', true)} on $\ell$. Note that since $d$'s \wwm{} linearized before the first such read of the \texttt{docket}, the first call to \texttt{helpLive} must have already read $d$ in the docket in this case.
	By Lemma~\ref{lem:CasInLoop}, and since $d'$'s \texttt{helpLive} calls always execute a CAS on the \texttt{live} slot, after its second \texttt{helpLive} call during \texttt{compete(d', true)}, a value at least as recent as $d$ has been move from \texttt{docket} to \texttt{live}. If this value is not $d$, then $d$ was not in \texttt{docket} when that CAS read \texttt{docket} for its new value. If $d$ was never on \texttt{live}, then it became invisible, so its danger interval is over. If $d$ was on \texttt{live} at some point, then by the end of $d'$'s third \texttt{helpLive} call, it is either aborted or safe, since by Lemma~\ref{lem:liveRemovalStatus}, it would not have been removed from \texttt{live} otherwise. If it is in \texttt{live} during $d'$'s third \texttt{helpLive} call and not aborted, then $d'$ runs \texttt{d.helpDescriptor}, so $d$ must be safe or aborted after that.
	
	Case 3. $d$ was not returned in either lines~\ref{line:readDocket} or~\ref{line:readLive} of $d'$'s \texttt{compete(d', true)} call in any of its \texttt{helpLive} instances. Then $d$ was invisible after its \wwm{} linearized, so the lemma holds.
	%	\Naama{To be adjusted.}
	%	Note that if $d$ threatens $d'$ and $d'$'s \activeInt{} started after $d$'s threat int, then, by Claim~\ref{clm:univ}, $d$'s wwm linearizes by $d'$'s \firstcritread{} on all locks. Clearly, this is also the case if $d$ was returned in $d'$'s \firstcritread.
	%	% returns from Line~\ref{line:linWWM} on all locks.
	%	%before $d'$'s wwm on all locks. 
	%	
	%	Note that the definitions of \firstcritread, \firstsuccCAS, and \assocClear{} remain identical between the single and nested versions of the algorithm. Therefore, exactly like in the single-lock case, if a descriptor $d$'s wwm is linearized before the \firstcritread{} of a descriptor $d'$ on the same lock, then $d$'s \firstcritread, \firstsuccCAS, and \assocClear{} on that lock must all be before or at the same time as the corresponding milestones of $d'$.
	%	
	%	In particular, this means that on every lock $\ell$ on which both $d$ and $d'$ contend, $d$'s \assocClear{} happens at the same time as or before $d'$'s \assocClear.  \Naama{For this, we assume \assocClear{} is one of the boundaries for threat interval. Must change argument if we change that.}
	%	
	%	We now consider the second case, in which $d$ was returned in $d'$'s \firstcritread. Note that in this case, $d$'s \firstcritread{} is the same as $d'$'s \firstcritread, since, by definition, if a descriptor is returned by any critical read, that read must be its \firstcritread. Therefore, by the definition of \firstsuccCAS{} and \assocClear, $d$ and $d'$ share those milestones as well. 
	%
	%\Naama{If $d$ was on the live slot at some point during $d'$'s execution on the same lock, then $d$ will be done on all its locks before $d'$. However, what if $d$ lost, and was never on live? Then $d'$ wouldn't have forced $d$ to terminate on all locks. What do we do then?  Maybe we can argue this only biases the probabilities in a good direction, i.e. giving the next $d'$ more of a chance to win, because $d$'s priority had to have been small.}
	%\Naama{New idea: what if we make the threat interval be until clear or abort? Does that work? No, doesn't work because you can get aborted by someone who is already aborted.}
	%  if two \op{s} have the same \firstcritread, then they have the same \firstsuccCAS{} and \assocClear{} as well. Furthermore, if an \op{} $op_1$'s \firstcritread{} is before another \op{} $op_2$'s \firstcritread, then $op_1$'s \firstsuccCAS{} and \assocClear{} must be either before those of $op_2$ or at the same time as those of $op_2$. 
	%
	%\Naama{To be slightly adjusted.}
	%Let $op_1$'s \firstcritread{} be at time $t_2$, and let $op_2$'s \firstcritread{} be at time $t_2$.
	%Furthermore note that by definition, $op_1$ threatens $op_2$ if and only if $t_1 \leq t_2$. Therefore, as argued above, $op_1$'s \assocClear{} must also be earlier or at the same time as $op_2$'s \assocClear.
\end{proof}


\begin{lemma}\label{lem:threatAbort}
	A descriptor $d$ can be \texttt{aborted} only if there is a threatener of $d$, $d'$, whose priority is higher than $d$'s priority.
	%, whose \activeInt{} overlaps with $d$ at least one of the following points on some lock $\ell$ that both $d$ and $d'$ accessed :
	%	\begin{itemize}
	%		\item the point at which $d$'s wwm linearizes on $\ell$
	%		\item the first time at which $d$ is invisible on $\ell$ after its wwm's linearization point.
	%		%the \texttt{docket} is read on Line~\ref{line:readDocket} in a \texttt{helpLive(d)} call
	%		\item the first time the check on Line~\ref{line:checkPriority} passes, while $d$ is the \texttt{liveVal} %on \texttt{live} %Line~\ref{line:tryAbortLock}
	%		\item the first time the check on Line~\ref{line:checkPriority} fails, while $d$ is the \texttt{dockVal} and \texttt{dockVal.tryAbort} is subsequently called in the same \texttt{helpLive} instance. % on \texttt{docket}
	%	\end{itemize}.
\end{lemma}

\begin{proof}
	Consider a descriptor $d$ whose status gets changes to \texttt{aborted}. There are three places in the code in which this can happen; on Line~\ref{line:abortNotInDocket}, Line~\ref{line:tryAbortLock} and on Line~\ref{line:abortDocket}. 
	% \Naama{Would become 3 or 4 places, depending on whether we leave in the aborting in helpDescriptor.}
	
	%We first note that the \texttt{tryAbort} call that successfully changes $d$'s status to \texttt{aborted} must have been executed during $d$'s danger interval, since $d$'s danger interval would end immediately after that \texttt{tryAbort}.
	% ends at the CAS that attempts to change its status to \texttt{safe}. If that CAS already happened, then $d$'s status can no longer be \texttt{active} (by Lemma~\ref{lem:noStatusChange}), and therefore the \texttt{tryAbort} would fail to change it. \Naama{Argument would change here if we change danger interval to end at abort, but it still works.}
	
	If the \texttt{tryAbort} that changed $d$'s status was executed on Line~\ref{line:abortNotInDocket}, then $d$ was not in the \texttt{docket} of one of its locks after its \wwm{} linearized, and before 
	it left the \texttt{active} status.
	%its \assocClear.
	Therefore, there must have been some other descriptor $d'$ whose priority was higher than $d$'s priority and was not yet aborted or safe at the time of either its \wwm{} or $d$'s \wwm{} on the \texttt{docket}. Thus, $d$'s danger interval overlapped with that of $d'$, and the lemma is satisfied.
	% If $d'$'s was ready at the time $d$'s \wwm{} linearized, then we are done. Otherwise, $d'$ must have set its ready flag to true after $d$'s wwm linearized. So, the first time that $d'$
	%Therefore, $d'$ threatened $d$, had a higher priority, and was active at one of the points outlined in the lemma statement.
	
	If the \texttt{tryAbort} that changed $d$'s status was executed on Line~\ref{line:tryAbortLock} by process $p$, then the descriptor $d' =$\texttt{dockVal} has a higher priority that $d$ and was not aborted at Line~\ref{line:checkPriority}, when $d$ was on the \texttt{live} slot but not yet aborted. Therefore, if $d'$ was also not safe at that time, then $d'$ satisfies the lemma. If $d'$ was safe at that time, note that $d = liveVal \neq dockVal$, since by assumption, $d$ eventually aborts, so it canont be safe by Lemma~\ref{lem:noStatusChange}. Furthermore, by Lemma~\ref{lem:safeHoldsLocks}, $d'$ must have been on the \texttt{live} slot of this lock before it became safe. For $d$ to get to \texttt{live} afterwards, it must have been read from \texttt{docket} after $d'$ was on \texttt{live}. Furthermore, $d'$ could only have been placed in \texttt{live} if it was on the docket before that. However, since $d'$'s \wwm{} can only linearize once, $d'$ can't be on the docket twice. Therefore, $d'$ cannot be safe.
	
	If the \texttt{tryAbort} that changed $d$'s status was executed on Line~\ref{line:abortDocket}, then the descriptor in \texttt{liveVal} must have had a higher priority and not been safe or aborted (by Line~\ref{line:checkPriority}, if \texttt{liveVal}'s priority was lower then it would have had tryAbort executed on it, and by the later checks, \texttt{liveVal} was not aborted or safe). Therefore, \texttt{liveVal} threatened $d$ and had a higher priority.
	%	there was some descriptor $d'$ whose priority was higher than $d$'s priority, and which was in the \texttt{docket} of one of $d$'s locks during the time $d$ was in the \texttt{live} slot of the same lock.  \Naama{Need to only try to abort the \texttt{live} if the dockVal isn't aborted yet. Add that check. Then this is easy.}
	%	%Note that this means $d'$'s \firstsuccCAS{} hadn't been executed yet on this lock at the time that $p$ read $d'$ in the \texttt{docket}. 
	%	Therefore, $d'$'s threat interval overlapped with $d$'s danger interval. 
	%	%\Naama{Might be a problem if threat interval ends when you get aborted. Would need to prevent a descriptor from kicking someone out of live if that descriptor is already aborted. Seems like too big a change in the algorithm.} 
	%	Thus, $d'$ is a threatener of $d$ whose priority is higher than $d$'s, satisfying the lemma.
	%	
	%	Finally, if the \texttt{tryAbort} that changed $d$'s status was executed on Line~\ref{line:abortDocket}, then there was a descriptor $d'$ in the \texttt{live} slot of one of $d$'s locks such that  $d'$'s priority was higher than $d$'s priority and $d'$ was not aborted at that time. \Naama{Need to check where the liveVal has aborted. Furthermore, why hasn't its \assocClear{} already happened? Maybe want to change boundary of threat interval a bit.}
	%	%
	%%	Otherwise, if the \texttt{tryAbort} that changed $d$'s status was executed on Line~\ref{line:abortself} by some process $p$, then $d$ was not in the \texttt{live} slot of one of its locks after $p$ competed on that lock. Let that lock be $\ell$. Note that $p$ must have competed on $\ell$ after $d$'s wwm was linearized on $\ell$, since $p$ ensures $d$'s wwm linearizes in $d$'s\texttt{helpDescriptor} before executing the compete, and before Line~\ref{line:abortself}. Since, by assumption, $p$'s \texttt{tryAbort} on Line~\ref{line:abortself} succeeded, $d$'s status must have been \texttt{active} immediately beforehand. By Lemma~\ref{lem:noStatusChange}, $d$'s status could not have been anything but \texttt{active} at any earlier point in time. By Lemma~\ref{lem:liveRemovalStatus}, since its status was \texttt{active}, $d$ could not have been in the \texttt{live} slot of $\ell$ at an earlier time and been removed. Therefore, $d$ was never in the \texttt{live} slot of a lock on which the compete function has been executed after $d$ announced its priority. Therefore, $d$'s \firstsuccCAS{} had a different descriptor $d'$ as its new value. By Lemma~\ref{lem:nested-blame}, $d'$ is a threatener of $d$ with a higher priority.
\end{proof}

\begin{lemma}\label{lem:winIfHighest}
	$d$'s thunk gets executed if $d$'s priority is the highest of all its threateners on all locks.
\end{lemma}

\begin{proof}
	%	If $d$'s priority is not the highest of all of its threateners, then let $d'$ be a descriptor that threatens $d$ and has a higher priority. We consider two cases. 
	%	If it's not max, then at some point it gets aborted. Aborted descriptors don't get their thunks executed.
	%
	By Lemma~\ref{lem:threatAbort}, if $d$ has the highest priority of all of its threateners, then it cannot be put in the \texttt{aborted} status. Therefore, eventually, some process (possibly the one that called the \texttt{tryLocks} instance that created $d$) will execute Line~\ref{line:tryProtect} in \texttt{d.helpDescriptor}, and succeed in changing $d$'s status to \texttt{safe}. By Lemma~\ref{lem:noStatusChange}, $d$'s status will remain \texttt{safe} once it becomes \texttt{safe}. Therefore, at some point in time, some process will successfully pass the check on Line~\ref{line:safeCheck}, and proceed to execute the thunk on Line~\ref{line:runThunk}.
\end{proof}




%Let $S$ be a schedule determined by the oblivious adversary. Depending on the realizations of the randomness, a descriptor $d$'s interval could end at different points during $S$. We now claim that if $d$ eventually becomes \texttt{safe}, its threat interval ends no later than its \activeInt{} in any realization in which $d$ eventually becomes \texttt{aborted}.

%\begin{lemma}\label{lem:WinShorterThanLose}
%	Given any schedule $S$ determined by the oblivious adversary, let $R_s$ be a realization of $S$ in which $d$ eventually becomes \texttt{safe}, and $R_a$ be a realization in which $d$ eventually becomes \texttt{aborted}. $d$'s  \activeInt{} in $R_s$ ends no later than its \activeInt{} in $R_a$.
%	%in every realization of $S$ in which descriptor $d$ eventually becomes \texttt{safe}, its threat interval ends earlier than its \activeInt{} does in every realization of $S$ in which if its thunk gets executed is no longer than its \activeInt{} if its thunk does not get executed.
%\end{lemma}
%
%\begin{proof}
%	
%	\Naama{General idea: doing your helpAll() takes the same amount of time regardless of how much contention there is. So, the only thing that matters is how many people you help. Need to argue that you must help more people if you get aborted than if you are safe. Should be able to argue per person you encounter: if you help when you don't abort, you must have also helped if you did abort.}
%\end{proof}
%
%\begin{lemma}\label{lem:nested-point-contention}
%	The number of descriptors that threaten a given descriptor $d$ is at most $2Pt$, where $Pt$ is $d$'s point contention.
%\end{lemma}
%
%\begin{proof}
%	Let $t$ be the time at which $d$'s ready flag was set to true (thus starting its \dangerInt), and let $t'$ be the time at which $d$'s first \texttt{tryProtect} was executed (ending its \dangerInt). Note that the number of descriptors that threatened $d$ is at most $Pt(t) + Pt(t') + \vert Fast \vert$, where $Fast$ is the set of descriptors that started their \activeInt{} after $t$ and finished their \activeInt{} before $t'$. 
%	
%	By Lemma~\ref{lem:nested-early-end}, if some descriptor $d'$ started its \activeInt{} after $d$'s threat interval (which is the same start time as its \dangerInt), then $d$'s \activeInt{} must end no later than $d'$'s on all the locks they share. Therefore, $Fast = \emptyset$.
%	Thus, the number of descriptors that threaten $d$ is at most  $Pt(t) + Pt(t') \leq 2Pt$.
%\end{proof}

\begin{lemma}\label{lem:nested-probs}
	The probability that a descriptor $d$ has the highest priority of
	all its threateners in an execution $E$ is at least $\frac{1}{2\kappa}$
	where $\kappa$ is point contention of $d$ in $E$.
\end{lemma}

\begin{proof}
	Let $t_s$ be the time at which $d$ begins its danger interval, and $t_e$ be the point at which $d$ finishes its danger interval. Note that by Observation~\ref{obs:wwm-indep}, $t_s$ does not depend on the priority of any descriptor. Note also that the start times of all the \activeInt{} of all descriptors do not depend on their priorities. Furthermore, by Lemma~\ref{lem:nested-early-end}, any descriptor $d'$ whose \activeInt{} starts after $t_s$ must end its \activeInt{} after $t_e$.
	
	Since there are at most $\kappa$ descriptors whose active interval overlaps any point, including $d$ itself, this means that there is a set $T$ of at most $2\kappa -2$ descriptors whose intervals overlapped at least one of $t_s$ or $t_e$, and this set is independent of the priorities of any of its descriptors, and the priority of $d$.
	Thus, the probability that $d$'s priority is higher than that of all descriptors in $T$ is the same as its probability to be the highest of $2\kappa-1$ uniform i.i.d random variables; $\frac{1}{2\kappa-1}$.
	
	Finally, since the danger interval of each descriptor is contained within its \activeInt, the set $T$ includes all of $d$'s threateners across all possible realizations on the randomness in execution $E$.
	%Consider the point in time, $t$ at which $d$ begins its danger interval, and the point in time $t'$ at which it ends its danger interval. By the definition of point contention, there are at most $\kappa$ descriptors whose \activeInt{} overlaps each of these points. 
\end{proof}

Lemmas~\ref{lem:winIfHighest} and~\ref{lem:nested-probs} immediately imply the following theorem about the fairness of the nested locks.

\begin{theorem}
	The probability that the thunk of a descriptor $d$ gets executed in an \op{} $a$ in execution $E$ is at least $\frac{1}{2\kappa}$ where $\kappa$ is point contention of $d$ in $E$.
\end{theorem}

%\begin{lemma}%\label{lem:nested-probs}
%	%The priorities of the threateners of a descriptor $d$ are distributed uniformly i.i.d..
%	The probability that a descriptor $d$ has the highest priority of all its threateners in an execution $E$ is  at least $1/(T*\kappa)$, where $T$ is the maximum number of threateners of $d$ in $E$, and $\kappa$ is $d$'s point contention in $E$.
%\end{lemma}
%
%\begin{proof}
%	Note that the priority of each descriptor is chosen uniformly at random from the same range, and independently of all other priorities. Furthermore, by Observation~\ref{obs:wwm-indep}, the number of steps it takes for a multi-location wwm operation to execute its \capture{} on all its locks is independent from the priority of that operation. Therefore, since the threat interval of descriptors starts once a descriptor has returned from \capture{} on all locks and set its ready flag to true, an oblivious adversary cannot influence the priorities of a descriptor $d$ before its threat interval start. 
%	%\Naama{Would need to change. Can no longer argue about beginning of threat interval, but maybe can argue about influencing threatener before and after the time of its ready flag.}
%	
%%	To complete the proof, consider a descriptor $d_t$ that threatens $d$. Note that by Lemma~\ref{lem:winShorterThanLose}, $d_t$'s \activeInt{} ends no earlier in this realization of the schedule than in a realization in which $d_t$ aborts. Furthermore, by Lemma~\ref{lem:threatAbort}, if $d$ aborts, then it must have overlapped with a descriptor whose priority was higher and   
%	
%	To complete the proof, we must also show that an oblivious adversary cannot influence the distribution of the priorities of threateners of $d$ by extending some threatener's interval depending on its priority. By Lemma~\ref{lem:WinShorterThanLose}, a threatener's \activeInt{} is no longer if it eventually becomes safe than if it eventually becomes aborted. In particular, in either case, and regardless of $d_t$'s priority, $d_t$'s \activeInt{} overlaps with $d$.
%	So, for every $d_t$, consider the point, $t$ at which $d_t$'s \activeInt{} intersects $d$'s \activeInt{} with the highest point contention. $d$ could not have had more threateners than $\kappa(t)$, for every actual threatener $d_t$ that it faced.
%	
%	Therefore, $d$'s probability of having the highest priority is at least $1/(T*\kappa)$.
%	\Naama{Make sure this proof is ok.}
%%	For this purpose, we show that if a descriptor $d$ is threatened by a descriptor $d_t$ on a lock $\ell$, the $d_t$ cannot be very biased toward a high priority. We prove this in two steps; first, we show that if $d_t$ caused $k$ other descriptors to be \texttt{aborted} on $\ell$, %that is blamed by $k$ other descriptors on a given lock $\ell$, 
%%	then $d$ is threatened by at least $k-1$ of these $k$ others.  Secondly, 
%	%We prove that if $d_t$ caused some other descriptor $d'$ to be \texttt{aborted}, then $d_t$'s threat interval is no longer than if it hadn't caused $d'$ to abort.
%	%\Naama{Problem: if we change definition of threaten to be wwm, then $d_t$ could be blamed on other locks and we might care. Key point in this proof is that $d_t$ starts threatening on all locks at once, so we can consider blames on each lock separately.} 
%	%
%%	For the first part,
%%	note that there are two reasons for $d_t$ to abort each of the $k$ descriptors, $d_1 \ldots d_k$; for each $d_i$, either $d_i$ was in the \texttt{live} slot of some lock $\ell$ when $d_t$ was in the \texttt{docket}, or $d_t$ was returned by $d_i$'s \firstcritread. 
%%	%By Lemma~\ref{lem:threatAbort}, all $k$ descriptors were threatened by $d_t$, and therefore, 
%%	By Lemma~\ref{lem:nested-early-end}, in the latter case, $d_t$'s threat interval cannot end after $d_i$'s threat interval. Thus, if $d_t$ threatens $d$, $d$ is threatened by $d_i$ as well. \Naama{If we change Lemma~\ref{lem:nested-early-end} to refer to \activeInt{} of the threatened desc, then $d$ won't be threatened by $d_i$, but would be concurrent with them at the time at which $d_t$ threatened $d$. So PtCtn would show up in the final bound, but that should be fine, as it should be additive.}
%%	
%%	We now consider the former case, in which $d_i$ was already in the \texttt{live} slot when it was aborted by $d_t$, and show that there can be at most one such $d_i$. Assume by contradiction that there can be several descriptors that were in the \texttt{live}  slot and were aborted while $d_t$ was in the \texttt{docket}. Note that after the first such descriptor is aborted, the \texttt{live} slot must change. The only way the \texttt{live} slot is changed is by CASing in a new value from the \texttt{docket}. This new value must either be $d_t$ itself, or some newer value that replaced $d_t$ in the \texttt{docket}. In either case, $d_t$ can no longer abort another descriptor in the \texttt{live} slot.
%%	
%%	Therefore, $d$ must be threatened by at least $k-1$ of these descriptors.
%%	Thus, $d$'s probability of having the highest priority of all of its threateners is its probability of having the highest of priority of $T+1$ uniform i.i.d random variables. \Naama{This would change to be T+ PtCtn+1, I think.}
%%	
%%	We now consider the second case, in which $d_t$ caused some descriptor $d'$ to abort on some other lock $\ell'$. Then, since $d_t$ threatens $d$, it could not have been aborted, and by Lemma~\ref{lem:abortBeforeHelp}, could not have helped any other descriptor before getting to lock $\ell$. Therefore, \Naama{since executing the wwm (and read on docket) always take the same number of steps,} and all other parts of the execution take a constant number of steps, $d_t$'s execution is at most as long as it would have been had it aborted. Therefore, $d$ would have contended with it in either case. \Naama{This leads to a PtCtn bound again, since we have to count not only the threateners, but also the ones in their \activeInt. But this one looks like $PtCtn \cdot T$, since I don't think there's a way to argue all the potential threateners had to overlap. This means that our final fairness bound would be $1/PtCtn^2$.} 
%%	
%%	\Naama{This entire lemma proof can be shrunk if we prove the previous lemma. But this proof is fine if we enforce access to the wwm object to always take the same amount of time. Seems to me like even with that lemma, the final bound would be $T\cdot PtCtn$}
%	%
%	%We now consider the second case, in which $d_t$ caused some descriptor $d'$ to abort on some other lock $\ell'$. Here, we again consider two cases, based on whether or not $d_t$ ended up being on the \texttt{live} slot of $\ell'$ at some point in time. If not, then $d_t$'s execution on $\ell'$ took exactly the same steps as it would have had it not caused $d'$ to abort. \Naama{verify this.} Therefore, its execution was not extended by the fact that it caused an abort.
%	%In the second case, if $d_t$ did get to the \texttt{live} slot, then \Naama{what then? Maybe we can count $d'$ as a `threatener' too, since it would have to still be active, so it is counted in our point contention?}
%%
%\end{proof}

%\begin{lemma}
%	Given the same set of competitors, the timing of $p$'s execution of the compete() function has no effect on whether its descriptor wins.
%\end{lemma}
%
%\begin{proof}
%	Anyone who executes compete() on any of $p$'s locks after $p$ announced its descriptor will execute exactly the same operations as $p$. Should be able to point to a lemma about the single lock to prove this.
%\end{proof}



%Therefore, putting Lemmas~\ref{lem:nested-point-contention} and~\ref{lem:nested-probs} together, we get that the algorithm for nested locks is \emph{fair}, in that the probability for a thunk to get executed is at least $\frac{1}{2Pt+2}$.

==> univProof.tex <==
\section{Analysis of the Universal Construction}\label{sec:univProof}

We begin by identifying a key point in time during the execution of an update operation.

\begin{definition}
	The \emph{reveal time} of an update by a process $p$ with descriptor $d$, denoted $t_{d}$, is the first time at which both (1) $d$ is announced in some slot of the announcement array, and (2) $d$'s ready flag is set to true.
\end{definition}

\begin{claim}\label{clm:univ}
	An update operation with descriptor $d$ by process $p$ gets linearized sometime between when $d$'s ready flag is set to true and when $p$ returns from the call to \texttt{update}.
	Furthermore, let $q$ be a process that started an instance of \texttt{helpAll} after time $t_d$. Then $p$'s update is linearized before $q$ returns from its \texttt{helpAll} call.
%	After process $p$ executes \texttt{update}, $p$'s operation has been applied to the object.
\end{claim}

To prove the above claim, we first show a few simpler lemmas.

\begin{lemma}\label{lem:announcementOwner}
	Once a process $p$ writes a non-null value into an announcement slot \texttt{Announce[i]}, no process other than $p$ can change the value in \texttt{Announce[i]} until after $p$ writes $null$ into the slot.
\end{lemma}

\begin{proof}
	Processes can modify an announcement slot \texttt{Announce[i]} in two places; using a CAS on line~\ref{line:grabslot}, and using a write on line~\ref{line:clearAnn}. The CAS on line~\ref{line:grabslot} always uses $null$ as its old value. Therefore, if the current value is not null, any such CAS would fail. Furthermore, note that the write on line~\ref{line:clearAnn} only gets executed by a process $q$ if $q$ succeeded in its CAS on line~\ref{line:grabslot} on that slot. Therefore, if a process $p$ writes a non-null value into \texttt{Announce[i]}, every other process $q$ would fail its CAS on line~\ref{line:grabslot} and subsequently not try to write a value  on line~\ref{line:clearAnn}. 
\end{proof}

\begin{lemma}\label{lem:successCAS}
	
	Consider any process $p$ updating the object with descriptor $d$. 
	%Let $t$ be the first time at which $p$'s descriptor was both (1) announced in some slot of the announcement array, and (2) its ready flag was set to true.
	Let $q$ be the first process that completed two calls to \texttt{help} such that both of the calls started after $t_{d}$, and let $t'$ be the time at which $q$ completed its second such \texttt{help} call.
	There must be a successful CAS $C$ on the \texttt{Current} object between $t_{d}$ and $t'$ such that $C$'s associated read is also executed between those times.
%	
%	executes line~\ref{line:grabslot} and the time at which it executes line~\ref{line:clearAnn}, such that $C$'s associated read is also executed between those times. \Naama{is `associated read' ok here? Maybe find a different term.}
%	\Naama{Change this to time at of call to first help instead of CAS. Doesn't change the proof.}
\end{lemma}

\begin{proof}
%	Note that a process $p$ updating the object calls \texttt{help} twice between the time, $t$, at which it executes line~\ref{line:firsthelp} and the time, $t'$ at which it executes line~\ref{line:clearAnn}. 
	
	By the definitions of $t_{d}$ and $t'$, there must have been two calls to \text{help} between $t_{d}$ and $t'$ whose intervals did not overlap, executed by some process $q$.
	%
	Each call to \texttt{help} begins with reading the \texttt{Current} object on line~\ref{line:readCurrent} and ends with executing a CAS on the \texttt{Current} object on line~\ref{line:CAScurrent}. Therefore, $q$ executed two CAS instructions on \texttt{Current} between $t_{d}$  and  $t'$. 
	%$p$ itself executes two CAS instructions on \texttt{Current} between $t$  and  $t'$. 
	%
	If at least one of $q$'s CASes succeeds, then the lemma holds. So, consider an execution in which both of $q$'s CASes on \texttt{Current} fail. Note that each CAS can only fail because some other process executed a successful CAS on \texttt{Current} between $q$'s most recent read of \texttt{Current} on line~\ref{line:readCurrent} and its CAS. Since $q$ rereads \texttt{Current} between its CAS attempts, two distinct CAS instructions by other processes must have  been executed. Denote these two CASes as $C_1$ and $C_2$, where $C_1$  happens before $C_2$  in the execution. Consider the read $R_2$ of \texttt{Current} associated with $C_2$. Note that $C_1$ must have  happened before $R_2$, since otherwise $C_1$ would have caused $C_2$ to fail. Note also that $q$'s initial read of \texttt{Current}, $R_{q,1}$ happens before  $C_1$, since otherwise $C_1$ would not have caused the failure of $q$'s first CAS. Therefore, we have the following happens before relationships: $t_{d} <_H R_{q,1} <_H C_1 <_H R_2 <_H C_2 <_H t'$. Therefore, $C_2$ is a successful CAS that happened between $t_{d}$ and $t'$, whose associated read also happened between those times.
\end{proof}

%\begin{lemma}\label{lem:flagmismatch}
%	While \texttt{Announce[i].flag == Current.flags[i]}, \texttt{Current.flags[i]} cannot change.
%\end{lemma}
%
%\begin{proof}
%	content...
%\end{proof}


\begin{lemma}\label{lem:rightflags}
	For any index $i$, while \texttt{Announce[i] == null}, \texttt{Announce[i].flag == Current.flags[i]}.
\end{lemma}

\begin{proof}
	The proof is by induction on the number of times a value has been announced in slot $i$ in an execution $E$.
	
	\textsc{Base.} Consider an execution $E$ in which slot $i$ has had no values announced in it. Note that the flags are initialized such that  \texttt{Announce[i].flag == Current.flags[i]} at the beginning of the execution. For \texttt{Announce[i].flag} to change, a process must announce a non-null value in \texttt{Announce[i]}, which, by  assumption, does not happen in $E$. For \texttt{Current.flags[i]} to change, a process must have changes this value in a CAS in line~\ref{line:CAScurrent} in the \texttt{help} function. However, any process executing \texttt{help} will have read \texttt{null} in \texttt{Announce[i].update}, and therefore failed the check on line~\ref{line:ifNeedsHelp}, and not modified \texttt{Current.flags[i]}. Therefore, \texttt{Announce[i].flag == Current.flags[i]} in $E$.
	
	\textsc{Step.} Assume that the claim holds in any execution in which a value is announced in slot $i$ up to $k$ times . Consider an execution $E$ in which $k+1$ values have been announced in slot $i$. Let $t_{k+1}$ be the time at which the $k+1$th value was announced on $i$. If the $k+1$th value is never cleared from slot $i$ in $E$, then note that the lemma holds on the prefix of $E$ including everything until right before time $t_{k+1}$ (by the induction hypothesis), and there are no more times in $E$ during which \texttt{Announce[i] == null}, so the lemma holds for $E$.
	
	So, assume that the $k+1$th value in slot $i$ does get cleared in $E$, and let $t_{k+1}'$ be the time at which the $k+1$th value was cleared.	
	Note that immediately after $t_{k+1}$, \texttt{Announce[i].flag != Current.flags[i]}, since by the induction hypothesis, \texttt{Announce[i].flag == Current.flags[i]} immediately before $t_{k+1}$, and by the algorithm, $p$ flips \texttt{Announce[i].flag} when it announces its update at time $t_{k+1}$.
	Furthermore, at time $t_{k+1}'$, $p$ does not flip \texttt{Announce[i].flag}. So, for the lemma to hold, we must show that \texttt{Current.flags[i]} gets flipped an odd number of times between $t_{k+1}$ and $t_{k+1}'$. We will show that this flag gets flipped exactly once during that interval.
	
	By Lemma~\ref{lem:successCAS}, there is some successful CAS on \texttt{Current} after $t_{k+1}$ and before $t_{k+1}'$ whose associated read on line~\ref{line:readCurrent} was also between those times. Let $C$ be the first such CAS, let $q$ be the process that executed $C$, and let $H$ be $q$'s execution of this instance of the \texttt{help} function. Note that $q$'s read of \texttt{Announce[i]} in $H$ must have returned the value written on it at time $t_{k+1}$, since it occurred before $t_{k+1}'$, and by Lemma~\ref{lem:announcementOwner}, no other value could have been written there during this time. 
	
	Note that any CAS executed on \texttt{Current} before $C$ whose associated read occurred after the previous value of \texttt{Announce[i]} was cleared would not have changed \texttt{Current.flags[i]}, since it must have read \texttt{null} in \texttt{Announce[i].update}. Then $q$'s new value must flip \texttt{Current.flags[i]}, since $q$'s check at line~\ref{line:ifNeedsHelp} must succeed;  immediately after $t_{k+1}$, \texttt{Announce[i].flag != Current.flags[i]},  \texttt{Announce[i].update !=null}, and $C$ is the first operation to change \texttt{Current} since $t_{k+1}$.
	
	We now argue that $C$ is the only successful CAS that changes \texttt{Current.flags[i]} until after $t_{k+1}'$. Assume by contradiction that some other CAS $C'$ does change \texttt{Current.flags[i]} after $C$ and before $t_{k+1}'$. Assume without loss of generality that $C'$ was the first such CAS. If $C'$ read \texttt{Current} on line~\ref{line:readCurrent} before $C$ was executed, $C'$ must have failed, contradicting the assumption that it was successful. Otherwise, $C'$ must have read values from both \texttt{Announce[i]} and \texttt{Current} such that it saw \texttt{Announce[i].flag == Current.flags[i]} in its check in line~\ref{line:ifNeedsHelp}, so it would not have changed \texttt{Current.flags[i]}. Contradiction.
%	\Naama{Might need to slightly modify proof to have executions in which the $k$th value has not been cleared in the induction hypothesis, and show it for an execution in which the $k+1$th value has not been cleared. Only a slight modification of notation, but I think it might be necessary to cover  the entire interval in which the announced value is null.}
%	
%	Therefore, neither \texttt{Announce[i].flag} nor \texttt{Current.flags[i]} can change between the time at which $C$ was executed and $t_{k+1}$, the time at which the $k+1$th update  was announced in \texttt{Announce[i]}. Since at the time $C$ was executed, \texttt{Announce[i].flag == Current.flags[i]} , and \texttt{Announce[i].flag} gets flipped at time $t+{k+1}$, the claim holds.
\end{proof}

\begin{lemma}\label{lem:linAfterReady}
	An update cannot get linearized before its descriptor's ready flag is set to true.
\end{lemma}

\begin{proof}
	Clearly, an update cannot be linearized if its descriptor is not written on some slot of the announcement array \texttt{Announce}. 
	Let $d$ be a descriptor written in \texttt{Announce[i]}. Note that $d$ can only get applied to the object if some process executed Line~\ref{line:applyUpdate} on \texttt{Announce[i]}, and then successfully executed the CAS on Line~\ref{line:CAScurrent}. However, for a process $p$ to execute Line~\ref{line:applyUpdate}, its check on Line~\ref{line:ifNeedsHelp} must pass; this check can't pass if $d$'s ready flag is set to false.
\end{proof}

We are now ready  to prove Claim~\ref{clm:univ}.

\begin{proof}[Proof of Claim~\ref{clm:univ}]
	Let $i$ be the index in which $p$ announces its update with descriptor $d$. By Lemma~\ref{lem:linAfterReady}, the update could not have been linearized before $p$ set its $d$'s ready flag to true. By Lemma~\ref{lem:announcementOwner}, \texttt{Announce[i]} must have been null immediately before the time, $t$, at which $p$ announced. By Lemma~\ref{lem:rightflags}, immediately before $t$, \texttt{Announce[i].flag == current.flags[i]}. By the algorithm, $p$ flipped \texttt{Announce[i].flag} at  time $t$, so immediately after $t$, \texttt{Announce[i].flag != current.flags[i]}. 
	
	%Let $t_{ready}$ be the time at which $p$ set its ready flag on this update.
	Let $q$ be a process that started a \texttt{helpAll} call %executing an update with descriptor $d'$, which started its update operation 
	after time $t_d$.
	By Lemma~\ref{lem:successCAS}, there is some successful read-CAS on \texttt{Current} that both occurred between $t_{d}$ and $t'$, where $t'$ is the next time at which some process executed two \texttt{help} calls that both started after $t_d$. Note that since, during the execution of an update and after a descriptor is announced and its ready flag is set to true, a process calls the \texttt{help} function twice, $t'$ is earlier than both $p$'s completion of its update and $q$'s completion of its helpAll.
	% finished its update and when $q$ finished its update.
	%
	%$p$ cleared its value from \texttt{Announce[i]} at time $t'$, whose associated read on line~\ref{line:readCurrent} was also between $t_{d}$ and $t'$. 
	Let $C$ be the first such CAS, let $s$ be the process that executed $C$, and let $H$ be $s$'s execution of this instance of the \texttt{help} function. Note that $s$'s  read of \texttt{Announce[i]} in $H$ must have returned the value written on it at time $t$, since it occurred before the value was cleared from \texttt{Announce[i]}, and by Lemma~\ref{lem:announcementOwner}, no other value could have been written there during this time. 
	
	Note that any CAS executed on \texttt{Current} before $C$ whose associated read occurred after the previous value of \texttt{Announce[i]} was cleared would not have changed \texttt{Current.flags[i]}, since it must have read \texttt{null} in \texttt{Announce[i].update}. Therefore $s$'s check at line~\ref{line:ifNeedsHelp} must succeed, since at time $t$ \texttt{Announce[i].update !=null} and \texttt{Announce[i].flag != Current.flags[i]}, and neither fields could have changed in the meantime. Thus, $s$ must have linearized $p$'s update, before either $p$ or $q$ completed.
\end{proof}

Finally, we make the following observation, which will be useful when arguing about the fairness of the nested lock construction we presented in Section~\ref{sec:nestedLock}.

\begin{observation}\label{obs:wwm-indep}
The linearization point of an update with descriptor $d$ does not depend on the content of $d$, other than its ready flag.
\end{observation}

\begin{proof}
	Processes applying the updates do not check the content of the descriptor before applying them to their local copy of the object. Furthermore, the success of the CAS on Line~\ref{line:CAScurrent} does not depend on the content of the new value, which is the only part that contains the effect of the update.
\end{proof}




==> unknownBound.tex <==
\section{Unknown Bound on Contention}\label{sec:unknownBound}
Here we present the pseudocode for the version of the lock algorithm that does not know the contention bound $\kappa$ and the bound on the number of locks per attempt, $L$. The lines in red are the ones that changed over the original version presented in Algorithm~\ref{alg:lock}.
\begin{figure}
\begin{lstlisting}
struct @\Descriptor@:
	lockList //list of active set objects
	thunk
	priority
	status = {active, won, lost}
	
	bool getFlag():
		@\red{return (priority > 0 || priority == TBD)}@
	void setFlag():
		@\red{Delay until total number of steps is the next power of two}@ @\label{line:delay1}@ 
		priority = @\red{TBD //participation reveal step }@
	void clearFlag():
		priority = -1

tryLocks(@\Descriptor@ p):
	p = new @\Descriptor@(lockList, thunk, -1, active)
	for each lock @$\ell$@ in p.lockList:
		set = getSet(@$\ell$@) 
		for each p' in set:
				run(p')
	multiInsert(p, p.lockList)
	@\red{numContenders =}@ run(p)
	multiRemove(p, p.lockList)
	@\red{Delay until $numContenders \cdot T$ steps taken since previous delay}@
	
@\red{int}@ run(@\Descriptor@ p): 
	@\red{Lock[] sets}@
	@\red{int numContenders = 0}@
	@\red{for each lock $\ell$ in p.lockList}@
		@\red{sets[$\ell$] = getSet($\ell$) }@ 
		@\red{numContenders += size(sets[$\ell$])}@
	@\red{CAS(p.priority, TBD, rand) //priority reveal step}@
	for each lock @$\ell$@ in p.lockList
		if (p.status == active): 
			for p' in sets[@$\ell$@]:
				if (p'.status == active): 
					if  p.priority > p'.priority: 
						eliminate(p')             
					else if (p != p'): eliminate(p) 
				celebrate(p')
	decide(p)  
	celebrate(p) 
	@\red{return numContenders}@
	
decide(@\Descriptor@ p):
	CAS(p.status, active, won)

eliminate(@\Descriptor@ p):
	CAS(p.status, active, lost)
	
celebrate(@\Descriptor@ p):
	if(p.status == won):
		execute p.thunk
\end{lstlisting}
\caption{Lock Algorithm}
\label{alg:lockUnknown}
\end{figure}

\subsection{Proof}

\begin{lemma}\label{lem:startThreatUnknown}
	Let $p$ and $p'$ be  \descriptor{s} such that $p$'s tryLock starts after $p'$'s participation-reveal step. Then neither \descriptor{} can cause the other to lose.
	%A process $p$ cannot cause a process $p'$ to fail if $p$ starts its tryLock attempt after $p'$'s reveal step.
\end{lemma}

The proof of this lemma is almost identical to the proof of its counterpart for the known-bound algorithm (Lemma~\ref{lem:threatStartcopy}).

\begin{proof}
	By Lemma~\ref{lem:differentLocks}, if $p$ and $p'$'s lock sets do not overlap, the lemma holds.
	Otherwise, if $p'$ has already removed itself from the active set by the time $p$ started its \code{getSet} on Line~\ref{line:getHelpSet}, then $p'$ must have already won or lost by this time. In particular, $p$ wasn't in the active set during $p'$'s \code{run(p')}, and therefore could not have caused $p'$ to lose. Furthermore, by Lemma~\ref{lem:endThreat}, $p'$ cannot cause $p$ to lose.
	
        So, assume that $p'$ is still in the active set at the time
        $p$ started its \code{getSet} on
        Line~\ref{line:getHelpSet}. By the set regularity of the multi active set algorithm,
       % linearizability of the active set algorithm \guy{[Reviewer complained about this. Should it be ``base'' active set algorithm'']}, 
      since $p'$ must have completed its
        insertion into the active set before $p$ started its
        \code{getSet} on Line~\ref{line:getHelpSet}, $p$ must have
        $p'$ in the set it gets. 
        %Furthermore, since $p'$ already revealed its participation (set its priority to \code{TBD}) before $p$'s \code{getSet} linearized, $p$ must see a non-negative or \code{TBD} priority for $p'$. 
        Therefore, $p$
        calls \code{run(p')} before its own participation-reveal step,
        so by Lemma~\ref{lem:doneStatus}, $p'$ wins or loses because
        of a different \descriptor{}. Furthermore, again by
        Lemma~\ref{lem:endThreat}, $p'$ cannot cause $p$ to lose,
        since a \code{run(p')} call completes before $p$'s reveal
        step, and therefore $p'$ is no longer active by that time.
\end{proof}

\begin{observation}\label{obs:threatUnknown}
	The set of \descriptor{s} whose intervals overlap a \descriptor{} $p$'s participation-reveal step includes all of $p$'s threateners.
\end{observation}

\begin{proof}
	Every \descriptor{} $p$'s interval includes a complete call to \code{run(p)}. Thus, by Lemma~\ref{lem:doneStatus}, the status of any \descriptor{} is not \code{active} by the end of its interval. The lemma is therefore immediately implied from Lemmas~\ref{lem:endThreat} and~\ref{lem:startThreat}.
\end{proof}

We can now prove the main theorem, using a similar argument to proof of the fairness theorem of the known-bound version. The main difference is that here, a \descriptor{} $p$'s participation reveal step is not completely predetermined at its start, but rather has $\log (\kappa L T)$ possible locations in the execution, where $C_p$ is the maximum contention $p$ can experience across its locks.

%\begin{theorem}
%	Let $k_\ell$ be the bound on the maximum point contention possible on lock $\ell$, and let $C_p = \sum_{\ell \in p.lockList} k_\ell$ be the sum of the bounds on the point contention across all locks in a \descriptor{} $p$'s lock list. Then the probability that $p$ succeeds in its tryLock is at least $\frac{1}{C_p\log C_p}$ in the lock algorithm that does not know the bounds $k_\ell$ (Algorithm~\ref{alg:lockUnknown}).
%\end{theorem}

\begin{theorem}
	Let $k_\ell$ be the bound on the maximum point contention possible on lock $\ell$, $\kappa$ be an upper bound on $k_\ell$ for all $\ell$, and let $C_p = \sum_{\ell \in p.lockList} k_\ell$ be the sum of the bounds on the point contention across all locks in a \descriptor{} $p$'s lock list. Furthermore, let $L$ be the maximum number of locks per tryLock attempt, and $T$ be the maximum length of a critical section. Then there exists an algorithm $A$ for wait-free fine-grained locks against an oblivious scheduler and an adaptive player such that (1) the probability that $p$ succeeds in its tryLock is at least $\frac{1}{C_p\log (\kappa L T)}$ in $A$, and (2) $A$ that does not know the bounds $k_\ell$, $\kappa$ and $L$. % (Algorithm~\ref{alg:lockUnknown}).
\end{theorem}

\begin{proof}
	At each of $p$'s $\log (\kappa L T)$ possible participation-reveal times, the adversary can make at most $C_p$ \descriptor{s} be potential threateners of $p$. Assume that the priority of each \descriptor{} $p'$ is picked uniformly at random at the beginning of the execution, but is hidden until after $p'$'s priority-reveal time. This matches our setting since priorities are always picked uniformly at random at the priority-reveal time.
	By Observation~\ref{obs:fixedAfterReveal}, the number of steps that a \descriptor{} $p'$ takes after its priority-reveal time until it terminates is determined before $p'$'s priority-reveal time. 
	Furthermore, note that the priority-reveal time of each of a \descriptor{} $p$'s potential threateners must be after $p$ starts, by Lemma~\ref{lem:startThreatUnknown}. Additionally, by this time, $p$'s participation-reveal time is fixed to be at one of $\log (\kappa L T)$ steps in the execution.
	Thus, before knowing $p'$'s priority, the adversary must decide which of $p$'s possible participation-reveal times $p'$'s interval will overlap. 
	Once the adversary decided this, it can reveal $p'$'s priority, and based on this, can decide whether to reveal other \descriptor{s}' priorities. However, by the arguments above, there are at most $C_p\log (\kappa L T)$ potential threateners of $p$ whose priorities it can reveal, and these priorities are all chosen uniformly at random. Therefore, $p$'s chance of success is at least the chance that its uniformly random priority is the highers of $C_p \log (\kappa L T)$ uniformly random i.i.d. values -- $\frac{1}{C_p\log (\kappa L T)}$.
\end{proof}

